Enhancing Next-Generation Extended Reality Applications with Coded Caching

The next evolutionary step in human-computer interfaces will bring forward immersive digital experiences that submerge users in a 3D world while allowing them to interact with virtual or twin objects. Accordingly, various collaborative extended reality (XR) applications are expected to emerge, imposing stringent performance requirements on the underlying wireless connectivity infrastructure. In this paper, we examine how novel multi-antenna coded caching (CC) techniques can facilitate high-rate low-latency communications and improve users' quality of experience (QoE) in our envisioned multi-user XR scenario. Specifically, we discuss how these techniques make it possible to prioritize the content relevant to wireless bottleneck areas while enabling the cumulative cache memory of the users to be utilized as an additional communication resource. In this regard, we first explore recent advancements in multi-antenna CC that facilitate the efficient use of distributed in-device memory resources. Then, we review how XR application requirements are addressed within the third-generation partnership project (3GPP) framework and how our envisioned XR scenario relates to the foreseen use cases. Finally, we identify new challenges arising from integrating CC techniques into multi-user XR scenarios and propose novel solutions to address them in practice.

==> 3D-WIDE-Text.tex <==
\subsection{Objectives and ambition}

An increasingly large share of today’s population is continuously connected to the virtual information world through mobile flat-screen devices, such as smartphones and tablets. The next step in the evolution of human-computer interfaces will bring forward immersive viewing experience facilitated by more capable wearable gadgets that submerge users to the three-dimensional (3D) digital world with six degrees of freedom (forward/back, up/down, left/right, yaw, pitch, roll) and allow them to interact with different virtual objects while remaining seamlessly integrated to the reality. Although the idea of digital immersion has been around for decades [Sutherland1965], its mass adoption was severely hampered by movement-restricting wired connections between the interfacing headsets and the external hardware. Due to this physical constraint and the low processing capabilities of the available hardware, immersive experience has remained a rather niche concept until 2018, when a whole new generation of powerful and affordable (priced at \$200) untethered headsets flooded the market.

In 2020, intelligent high-end head-mounted devices that can support immersive viewing applications are already offered and shipped by multiple hardware suppliers. Improved hardware and software capabilities support comfortable immersive user experience that requires spatial audio and high-rate (4K-and-beyond) streaming to create real sensory perception of the presence in a digital environment. These emerging application requirements necessitate powerful and agile external radio connections and impose stringent communication requirements that include extremely high throughput links to the processing unit (e.g., 400 Mbps of expected mean data rate, and up to 3.3 Gbps for ultimate 3D video [Han2017a]) and ultra-low over-the-air latencies (around 1ms) as the total motion-to-photon latency for the rendered image should be less than 15 ms [Doppler2017]. Failure to satisfy the above requirements leads to so-called cybersickness, which manifests as discomfort, disorientation, or nausea caused by human sensory conflict [Fulvio2019]. These constraining features of human perception result in much higher importance of the radio link reliability and stability for peak data rates than in the case of traditional 2D screens.

Already today, when modern 360-degree cameras can capture video of extremely high quality, the software market offers an enormous number of extended reality (XR) applications that exponentially engage more and more people. With the growing penetration levels and usage intensity, the actual deployment densities will create a situation that even the most advanced radio networks simply cannot handle. While a single localized application can be supported today by existing microwave technologies (e.g., by the latest IEEE 802.11ac standard released in September 2019, with the data rates up to 1 Gbps [NI2019]), the presence of multiple connected users will cause interference and, hence, detrimental degradation of the radio link quality, which compromises streaming or rendering and consequently destroys immersion in the entire network.

The only feasible solution to enable massive immersion networks is to exploit the extremely high frequency (EHF) spectrum available in millimeter-wave (mmWave) bands and take advantage of wide bandwidth and miniaturized antenna elements that enable complex multi-antenna systems and highly directional transmission. Anticipating that, some hardware vendors have already supplemented their headsets with mmWave wireless adapters. However, with the mmWave connectivity promise of high throughput and low delay on a point-to-point link, comes a series of specific challenges such as, for example, volatile channel quality, blockage effects, and complex 3D interference footprint. If not handled properly, these aspects will become a critical impediment to enabling future dense and dynamic immersive networks with unconstrained macro- and micro-scale user mobility. Against the existing connectivity and architecture solutions that are not yet capable of providing sufficient quality-of-immersive-experience, this project uniquely puts forward an emerging vision of mmWave-based mobile immersive viewing systems that will reliably provide seamless high data rates and low latencies as well as support extreme peak rates and ensure the reliability of future demanding XR applications. The main objective of the proposed research is to deliver a physical layer connectivity framework accounting for specific effects of directional mmWave connectivity and efficient utilization of the increasingly affordable in-device memory via multipoint coded caching (CC).

\subsection{Concept and methodology}

Our envisioned scenario assumes an XR or hyper-reality environment (educational, industrial, gaming, defense, social networking, etc.), where a large group of users is submerged into a network-based immersive application that runs on a high-end eyewear and, hence, requires heavy multimedia traffic and is bound to guarantee a required level of user experience quality throughout the operating theatre (see Fig. 1). The multimedia consumers are scattered across the area covered by the application and can move freely; their streamed data is unique and highly location- and time-dependent. All this multimedia content eventually rendered to be seen by the participants is user-specific and requires extremely fast updates with delays lower than the human perception thresholds. Notably, a large part of rich multimedia content for rendering a certain viewpoint is common among the users, which offers opportunities for efficient use of pooled memory resources through intelligent cache placement and network coded multicast content delivery mechanisms.
The interfacing eyewear devices are equipped with mmWave transceivers and remain connected to the network through multiple transmit-receive points (TRPs) that enable reliable communication via multi-connectivity schemes to provide improved resilience to random blockage as well as increased coverage and capacity in the area. As computation capabilities and form-factor constraints of wearable devices may not permit entirely local content processing, and at the same time, fully network-based solutions may not be possible any time soon (network delays are a few orders higher than acceptable values for immersive experience [Han2017]), the only viable option to provide continuous quality of immersive experience remains in the use of the network edge infrastructures and/or in disseminating some of the data across the network via multipoint multicast beamforming of network coded content as well as employing proximate device-to-device connections (D2D) for direct content exchange.

A possibility of caching at the user devices and computation offloading onto the network edge opens perspectives to deliver high-throughput/low-latency traffic and provide high stability and reliability of radio connections for a truly immersive experience. The fact that modern mobile devices continue to grow the amounts of available storage (one of the cheapest network resources) makes (coded) caching especially beneficial given the uniqueness of our use case, where the popularity of limited and location-dependent content becomes much higher than in any traditional network. When user devices are in the proximity of a certain TRP, which acts as a “data shower” or a “data kiosk”, line-of-sight (LoS) multiple-input multiple-output (MIMO) links with extremely high throughput enable dynamic (re-)placement (almost free of cost) of cached content, which repeats itself for more relevant multimedia content when the group of users approaches another TRP.

Recognizing the inherently mobile nature of the emerging immersive systems and their content-centric location-specific landscape, we formulate the following hypotheses. Our basic hypothesis 1 is rooted in the fact that human body is a redundant system and no matter how random and unpredictable the human motion may seem, ultimately, the trajectories of worn devices (i.e., eyewear) even w.r.t. the six degrees of freedom (6DoF), demonstrate certain patterns. Our basic hypothesis 2 envisages a possibility to transmit/exchange by large chunks of shared multimedia content, which will be locally adapted/rendered to the specific 6DoF position of the target user. Our working hypothesis is in that exploiting statistical motion patterns as well as advanced content distribution and caching algorithms can dramatically increase the system performance, especially in wireless bottleneck areas with limited wireless connectivity. The proposed methodology will be applied to demonstrate the desired optimization mechanisms on all levels of the envisioned network to result in breakthrough insights on the most impactful system factors and constraints, fundamental limits, and in general, effective design principles of future immersive networks.

The core challenges of our use case are three-fold. First, wearable safety concerns due to their proximity to the skin and other human body tissues result in tight radiation, energy efficiency, and computation power constraints, which require minimizing the exposure time not only for the owner but also for other participants. The second specific aspect is dictated by unconstrained and generally unpredictable human mobility in full immersion use cases, which is more challenging to handle than in the case of smartphones, tablets, or low-end virtual reality headsets. The third group is brought by immersive 6DoF environments and includes requirements on the data rate, latency, and reliability, which, in our case, are followed by mmWave carrier challenges (e.g., inconsistent 3D coverage, unpredictable blockage, and limits of far-field assumptions for short-range MIMO links).

\subsection{Background part}

Background on coded caching: The pioneering work [Maddah-Ali2014] considers an information-theoretic framework for the caching problem and proposes a novel CC scheme, where instead of replicating high-popularity content near-or-at end-users, different contents are spread across different caches. The CC scheme [Maddah-Ali2014] has been extended to other setups such as online CC, hierarchical CC, and multi-server scenarios [Shariatpanahi2016]. In [Shariatpanahi2017], joint design of CC and zero-forcing (ZF) was proposed to benefit from the spatial multiplexing gain and the global gain of CC, at the same time. Moreover, generic multigroup multicast beamformer design solutions without the caching component were developed [Venkatraman2017]. In our target use case, if users are requesting different content, the BS can multicast the missing fragments assuming beforehand that the users subtract their locally known portion of the message. This provides an additional degree-of-freedom gain due to CC and, hence, reduces the delivery time (i.e. enables higher rate) as multiple users can be served simultaneously, interference-free. For further DoF gain, multiple groups can be served simultaneously, using more complex interference coordinations.

Preliminary results on multi-antenna coded caching: In [Tölli2018, Tölli2020], we proposed a joint design of coded caching (CC) and multigroup multicast beamforming to benefit from spatial multiplexing gain, improved interference management and the global CC gain, simultaneously. A major practical impediment of CC is that the number of packets, which each file should be split into, known as subpacketization, grows exponentially with the network size [Lampiris2018]. In [Salehi2019], we provided a new delivery scheme that enables the level of subpacketization to be selected freely among a set of predefined values depending on the basic network parameters such as antenna and user count. The numerical examples demonstrated that larger subpacketization generally results in better efficiency index and higher symmetric rate, while smaller subpacketization incurs a significant loss in the achievable rate. This enables more efficient caching schemes, tailored to the available computation/power resources. In [Mahmoodi2019], we addressed D2D-aided beamforming for coded caching in finite SNR regime, where the downlink phase utilizes multicast beamforming to serve all users and fulfill the remaining content demand simultaneously.

Proposed research, Task 2.1: Proactive location-dependent cache placement: Since in our use case users move with no constraints and request their data continuously, we will refer to a location-dependent probability distribution. We will investigate solutions that opportunistically fill the cache memory of the users with the data (e.g., multimedia content relevant to fixed structures of the virtual world) which is likely to be requested at a location with a weaker signal strength (i.e. a location with wireless bottleneck). The aim is to design cache placement such that, in such bottleneck scenarios, a significant portion of the multimedia content rendered on the eyewear is originated from the local cache available at the user terminal. On the contrary, less cache involvement is needed when the wireless connectivity is strong (closer to the TRPs). We will study a possibility of using mobility prediction to design efficient content cache placement methods. We will also explore various cache placement opportunities to establish appropriate schemes of distributing files across the selected cache memories w.r.t. the typical user movement patterns.

Proposed research, Task 2.2: Content delivery mode selection between D2D and CC multicast/unicast beamforming: In our scenario, we ‘compress’ the conventional caching timeline by assuming “peak/off-peak hours” to be on the order of minutes or even seconds. After the cache (re-)placement carried out using methods developed in Task 2.1, the network can potentially offload the requested content onto the D2D connections by utilizing the caches of the nearby users, especially in the case of a wireless bottleneck. If the local cache content is known at the network, the requests can be redirected to devices holding the content or parts of it. As the BSs oversee the request redirection, the D2D connections can be scheduled based on these content requests. We will consider the content delivery mode selection problem where the network decides whether it shares the content directly, possibly to multiple users simultaneously using unicast or CC multicast beamforming (as detailed in Task 1.2), or allocates the request to a short-range D2D connection. We will study hybrid scenarios when some of the content can be served by the network and other parts via the direct exchange. We will address discrete mode selection problems (integer problems that are generally NP-hard and require relaxation to reformulate them as continuous and practically solvable problem), similarly to [Tölli2016]. We will also estimate the practical gains of CC depending on the actual immersive network topology.

==> EnhancedXR_old.tex <==
We need a new framework to apply CC techniques to our envisioned XR scenario. In this regard, we split the application environment into several zones, and then, further split each zone into several single view areas (SVA). 
%This process is illustrated in Figure~\ref{fig:zoning}.

\noindent\textbf{Single view area.}
The definition of SVA is tied with content files; the static view of each SVA can be rendered using a dedicated content file. The shape and size of SVAs depend on the chosen rendering and process split model. For example, if all the process is done at the network edge (i.e., the XR device only displays the received image), one would need a 3D arrangement of SVAs such that one separate SVA is defined for every user location and her/his head orientation. However, if an omnidirectional 3D image is sent to the user based on her/his location and final corrections are made at the device, the SVA map could be defined by splitting the zone area into equal-sized square tiles. As discussed in~\cite{3GPPRef}, each rendering and process split model has its cons and pros in terms of the required bandwidth, delay sensitivity, and the device cost.

\noindent\textbf{Zoning.}
Users in the same zone cache (parts of) the content files associated with every SVA in that zone. Zoning is done such that the users pass through a high-data-rate region as they move between the zones so that they can update their cache contents, with a minimal communication cost, with the data that is foreseen to be requested in the new zone.

In Figure~\ref{fig:zoning}, we have illustrated zones and SVAs for an example XR scenario where five multi-antenna transmitters cooperatively deliver data to the requesting users. As users move from one zone to another, they pass through high-data-rate regions (the white area between zones), and hence, can update their cache contents without affecting the QoE of other users. It is also assumed the rendering is done at edge servers and the final correction is performed at the user device, resulting in a square-tile SVA map. 

%The users make requests at any instant following their SVA location at that instant. The transmitters then use coded caching techniques to deliver data to the users in the same zone with a high data rate and low latency.


%The first step in applying coded caching techniques to the envisioned XR scenario is to split the application environment into several \textit{zones}.
%Users within each zone cache (parts of) the contents that might be requested in that zone. Hence, coded caching techniques can be used to deliver requested data to the users in the same zone. Zoning should be done such that the users pass from an area with very high achievable data rate, to be able to update their cache contents with almost zero communication cost, as they move between every two adjacent zones. 
%according to the available cache memory and transmitter location(s). Users inside the same zone cache parts of every content that might be requested within that zone, and hence, can benefit from collaborative coded delivery of their requested contents. Zoning should be done such that the users pass through the proximity of at least one transmitter (i.e., an area with very high achievable rate) while moving between two adjacent zones, so that they are able to update their cache contents. This is because the cache contents of the users need to be updated as they enter a new zone, e.g., via passing through an area with high data rate availability (data shower).

With the definition of zones and SVAs, we can use CC techniques to increase the perceived communication rate.
%After splitting the XR application area into zones and defining SVAs in each zone, we can use coded caching techniques to increase the perceived communication rate. 
At specified time intervals, every user in the application environment requests a content file according to the instantaneous location (and orientation). Then, for every group of users in the same zone, the edge server creates a set of codewords and multicasts them following an underlying CC scheme. Every codeword simultaneously delivers data to a subset of target users (e.g., as illustrated in Figure~\ref{fig:cc_illustration}), thus multiplying the effective rate by the target group size.

%After splitting the XR application area into zones and defining SVAs in each zone, we can use coded caching techniques to increase the perceived communication rate. At specified time intervals, every user in the application environment requests a content file according to his/her instantaneous location (and orientation). Then, for every group of users in the same zone, the edge server creates a set of codewords and multicasts them following an underlying coded caching scheme. Every codeword simultaneously delivers useful data to a subset of target users (e.g., through the process illustrated in Figure~\ref{fig:cc_illustration}), thus multiplying the effective rate by the target group size.

It should be noted that, although zoning allows allocating larger cache portions to each cached file (as it limits the number of files by constraining the physical area), it does not necessarily increase the achievable coded caching gain. This is because the caching gain is proportional to the total cache size available in all the users~\cite{maddah2014fundamental}, and the zoning limits the effective number of users participating in the CC process. Nevertheless, zoning is beneficial as it reduces the chance of simultaneously serving users with very diverse channel conditions, hence avoiding the so-called near-far issue. Moreover, the complexity of CC algorithms is reduced as fewer users participate in a cache-aided data delivery session.

%The next step is to split each zone area into several single view areas (SVA), such that the static view at each SVA can be rendered with a single file. The shape and size of SVAs depend on the chosen rendering and process split model. If all the rendering and process is done at the edge and the XR device only displays the received image, one would need a 3D arrangement of SVAs such that one separate SVA is defined for every user location and his/her head orientation. However, as more processing is expected to be carried out at the XR device, a smaller number of SVAs is needed. For example, if an omnidirectional 3D image is sent to the user based on his/her location, and the final viewport is rendered at the XR device based on the head orientation, the SVA map would be defined by splitting the zone area into equal-sized square tiles. As discussed in~\cite{3GPPRef}, each rendering and process split model has its benefits and drawbacks in terms of the required bandwidth, delay sensitivity, and the device cost.

\rev{For clarification, theoretical gains resulting from CC techniques in some example single-zone XR setups are provides in Table~\ref{tab:my_label}. This table highlights why CC could be an exciting solution for future XR setups: it enables a large performance gain under realistic assumptions and this gain scales with the number of users. This is in contrast to many other communication techniques where the performance is primarily deteriorated as the number of users scales.}

%\todo[inline]{We can put the table here. It should be emphasized that the numbers are theoretic. Update: we cannot put the table here, as we need to describe the framework first.}






==> Figures/Dynamic_Data_1.tex <==
UCY	MCY	UCXSD	MCXSD
0.667	1	0	0
0.667	1	.1	0.1
0.667	1	.2	0.2
0.667	1	.3	0.3
0.667	1	.4	0.4
0.667	1	.5	.5
0.667	1	.6	.6
0.667	1	.7	.7
0.667	1	.8	.8
0.667	1	.9	.9
0.667	1	1	1
0.667	1	1.1	1.1
0.667	1	1.2	1.2
0.667	1	1.3	1.3
0.667	1	1.4	1.4
0.667	1	1.5	1.5
0.667	1	1.6	1.6
0.667	1	1.7	1.7
0.667	1	1.8	1.8
0.667	1	1.9	1.9
0.667	1	2	2
0.667	1	2.1	2.1
0.667	1	2.2	2.2
0.667	1	2.3	2.3
0.667	1	2.4	2.4
0.667	1	2.5	2.5
0.667	1	2.6	2.6
0.667	1	2.7	2.7
0.667	1	2.8	2.8
0.667	1	2.9	2.9
0.667	1	3	3
0.667	1	3.1	3.1
0.667	1	3.2	3.2
0.667	1	3.3	3.3
0.667	1	3.4	3.4
0.667	1	3.5	3.5

==> Figures/Dynamic_Data_2.tex <==
DynamicX	DynamicY	UCX	UCY	MCX	MCY	Helper	DynamicXSD	UCXSD	MCXSD
11	0.7143	11	0.6429	11	1	0.1	3.3166	3.3166	3.3166
10.2	0.7143	10.2	0.6429	10.2	1	0.2	3.1937	3.1937	3.1937
9.8	0.7143	9.8	0.6429	9.8	1	0.3	3.1305	3.1305	3.1305
9.6	0.7143	9.6	0.6429	9.6	1	0.4	3.0984	3.0984	3.0984
9.4	0.7143	9.4	0.6429	9.4	1	0.5	3.0659	3.0659	3.0659
9.2	0.7143	9.2	0.6429	9.2	1	0.6	3.0332	3.0332	3.0332
9	0.7589	9	0.6429	9	1	0.7	3	3	3
10.8	0.7143	10.8	0.6429	10.8	1	0.8	3.2863	3.2863	3.2863
9.8	0.7143	9.8	0.6429	9.8	1	0.9	3.1305	3.1305	3.1305
9.2	0.7143	9.2	0.6429	9.2	1	1	3.0332	3.0332	3.0332
9	0.7143	9	0.6429	9	1	1.1	3	3	3
9	0.7143	9	0.6429	9	1	1.2	3	3	3
8.6	0.7143	8.6	0.6429	8.6	1	1.3	2.9326	2.9326	2.9326
8.4	0.7143	8.4	0.6429	8.4	1	1.4	2.8983	2.8983	2.8983
8.4	0.7143	8.4	0.6429	8.4	1	1.5	2.8983	2.8983	2.8983
8.2	0.7143	8.2	0.6429	8.2	1	1.6	2.8636	2.8636	2.8636
8	0.7589	8	0.6429	8	1	1.7	2.8284	2.8284	2.8284
9	0.7143	9	0.6429	9	1	1.8	3	3	3
8.8	0.7143	8.8	0.6429	8.8	1	1.9	2.9665	2.9665	2.9665
8.6	0.7143	8.6	0.6429	8.6	1	2	2.9326	2.9326	2.9326
8.2	0.7143	8.2	0.6429	8.2	1	2.1	2.8636	2.8636	2.8636
8	0.7143	8	0.6429	8	1	2.2	2.8284	2.8284	2.8284
8	0.7143	8	0.6429	8	1	2.3	2.8284	2.8284	2.8284
7.8	0.7143	7.8	0.6429	7.8	1	2.4	2.7928	2.7928	2.7928
7.6	0.7143	7.6	0.6429	7.6	1	2.5	2.7568	2.7568	2.7568
7.4	0.7589	7.4	0.6429	7.4	1	2.6	2.7203	2.7203	2.7203
7.4	0.7143	7.4	0.6429	7.4	1	2.7	2.7203	2.7203	2.7203
7.2	0.7589	7.2	0.6429	7.2	1	2.8	2.6833	2.6833	2.6833
8.4	0.7282	8.4	0.6429	8.4	1	2.9	2.8983	2.8983	2.8983
7.8	0.7282	7.8	0.6429	7.8	1	3	2.7928	2.7928	2.7928
7.6	0.7282	7.6	0.6429	7.6	1	3.1	2.7568	2.7568	2.7568
7.4	0.7282	7.4	0.6429	7.4	1	3.2	2.7203	2.7203	2.7203
7.2	0.7589	7.2	0.6429	7.2	1	3.3	2.6833	2.6833	2.6833
7.4	0.7282	7.4	0.6429	7.4	1	3.4	2.7203	2.7203	2.7203
7.2	0.7282	7.2	0.6429	7.2	1	3.5	2.6833	2.6833	2.6833
7	0.7282	7	0.6429	7	1	3.6	2.6458	2.6458	2.6458
6.8	0.7589	6.8	0.6429	6.8	1	3.7	2.6077	2.6077	2.6077
6.8	0.7282	6.8	0.6429	6.8	1	3.8	2.6077	2.6077	2.6077
6.6	0.7589	6.6	0.6429	6.6	1	3.9	2.569	2.569	2.569
7.2	0.7282	7.2	0.6429	7.2	1	4	2.6833	2.6833	2.6833
6.8	0.7282	6.8	0.6429	6.8	1	4.1	2.6077	2.6077	2.6077
6.6	0.7589	6.6	0.6429	6.6	1	4.2	2.569	2.569	2.569
6.6	0.7282	6.6	0.6429	6.6	1	0.1	2.569	2.569	2.569
6.4	0.7589	6.4	0.6429	6.4	1	0.2	2.5298	2.5298	2.5298
6.2	0.7589	6.2	0.6429	6.2	1	0.3	2.49	2.49	2.49
6	0.8163	6	0.6429	6	1	0.4	2.4495	2.4495	2.4495
9.6	0.7143	9.6	0.6429	9.6	1	0.5	3.0984	3.0984	3.0984
8.8	0.7143	8.8	0.6429	8.8	1	0.6	2.9665	2.9665	2.9665
8.6	0.7143	8.6	0.6429	8.6	1	0.7	2.9326	2.9326	2.9326
8.4	0.7143	8.4	0.6429	8.4	1	0.8	2.8983	2.8983	2.8983
8	0.7143	8	0.6429	8	1	0.9	2.8284	2.8284	2.8284
7.8	0.7143	7.8	0.6429	7.8	1	1	2.7928	2.7928	2.7928
7.8	0.7143	7.8	0.6429	7.8	1	1.1	2.7928	2.7928	2.7928
7.6	0.7143	7.6	0.6429	7.6	1	1.2	2.7568	2.7568	2.7568
7.4	0.7143	7.4	0.6429	7.4	1	1.3	2.7203	2.7203	2.7203
7.2	0.7589	7.2	0.6429	7.2	1	1.4	2.6833	2.6833	2.6833
7.2	0.7143	7.2	0.6429	7.2	1	1.5	2.6833	2.6833	2.6833
7	0.7589	7	0.6429	7	1	1.6	2.6458	2.6458	2.6458
8.2	0.7192	8.2	0.6429	8.2	1	1.7	2.8636	2.8636	2.8636
7.8	0.7192	7.8	0.6429	7.8	1	1.8	2.7928	2.7928	2.7928
7.6	0.7192	7.6	0.6429	7.6	1	1.9	2.7568	2.7568	2.7568
8	0.7282	8	0.6429	8	1	2	2.8284	2.8284	2.8284
7.4	0.7282	7.4	0.6429	7.4	1	2.1	2.7203	2.7203	2.7203
7.2	0.7282	7.2	0.6429	7.2	1	2.2	2.6833	2.6833	2.6833
7	0.7282	7	0.6429	7	1	2.3	2.6458	2.6458	2.6458
6.8	0.7589	6.8	0.6429	6.8	1	2.4	2.6077	2.6077	2.6077
7	0.7282	7	0.6429	7	1	2.5	2.6458	2.6458	2.6458
6.8	0.7282	6.8	0.6429	6.8	1	2.6	2.6077	2.6077	2.6077
6.6	0.7282	6.6	0.6429	6.6	1	2.7	2.569	2.569	2.569
6.4	0.7589	6.4	0.6429	6.4	1	2.8	2.5298	2.5298	2.5298
6.4	0.7282	6.4	0.6429	6.4	1	2.9	2.5298	2.5298	2.5298
6.2	0.7589	6.2	0.6429	6.2	1	3	2.49	2.49	2.49
7.2	0.745	7.2	0.6429	7.2	1	3.1	2.6833	2.6833	2.6833
6.8	0.745	6.8	0.6429	6.8	1	3.2	2.6077	2.6077	2.6077
6.6	0.745	6.6	0.6429	6.6	1	3.3	2.569	2.569	2.569
6.4	0.745	6.4	0.6429	6.4	1	3.4	2.5298	2.5298	2.5298
6.2	0.7589	6.2	0.6429	6.2	1	3.5	2.49	2.49	2.49
6.6	0.745	6.6	0.6429	6.6	1	3.6	2.569	2.569	2.569
6.2	0.745	6.2	0.6429	6.2	1	3.7	2.49	2.49	2.49
6	0.7589	6	0.6429	6	1	3.8	2.4495	2.4495	2.4495
6	0.745	6	0.6429	6	1	3.9	2.4495	2.4495	2.4495
5.8	0.7589	5.8	0.6429	5.8	1	4	2.4083	2.4083	2.4083
5.6	0.7589	5.6	0.6429	5.6	1	4.1	2.3664	2.3664	2.3664
6	0.745	6	0.6429	6	1	4.2	2.4495	2.4495	2.4495
5.8	0.745	5.8	0.6429	5.8	1	0.1	2.4083	2.4083	2.4083
5.6	0.7589	5.6	0.6429	5.6	1	0.2	2.3664	2.3664	2.3664
5.4	0.7589	5.4	0.6429	5.4	1	0.3	2.3238	2.3238	2.3238
5.2	0.8163	5.2	0.6429	5.2	1	0.4	2.2804	2.2804	2.2804
7.8	0.7357	7.8	0.6429	7.8	1	0.5	2.7928	2.7928	2.7928
7.2	0.7357	7.2	0.6429	7.2	1	0.6	2.6833	2.6833	2.6833
7	0.7357	7	0.6429	7	1	0.7	2.6458	2.6458	2.6458
6.8	0.7357	6.8	0.6429	6.8	1	0.8	2.6077	2.6077	2.6077
6.6	0.7589	6.6	0.6429	6.6	1	0.9	2.569	2.569	2.569
7	0.745	7	0.6429	7	1	1	2.6458	2.6458	2.6458
6.6	0.745	6.6	0.6429	6.6	1	1.1	2.569	2.569	2.569
6.4	0.745	6.4	0.6429	6.4	1	1.2	2.5298	2.5298	2.5298
6.2	0.745	6.2	0.6429	6.2	1	1.3	2.49	2.49	2.49
6	0.7589	6	0.6429	6	1	1.4	2.4495	2.4495	2.4495
6.4	0.745	6.4	0.6429	6.4	1	1.5	2.5298	2.5298	2.5298
6	0.745	6	0.6429	6	1	1.6	2.4495	2.4495	2.4495
5.8	0.7589	5.8	0.6429	5.8	1	1.7	2.4083	2.4083	2.4083
5.8	0.745	5.8	0.6429	5.8	1	1.8	2.4083	2.4083	2.4083
5.6	0.7589	5.6	0.6429	5.6	1	1.9	2.3664	2.3664	2.3664
5.4	0.7589	5.4	0.6429	5.4	1	2	2.3238	2.3238	2.3238
6.4	0.7627	6.4	0.6429	6.4	1	2.1	2.5298	2.5298	2.5298
6.2	0.7627	6.2	0.6429	6.2	1	2.2	2.49	2.49	2.49
6.2	0.7627	6.2	0.6429	6.2	1	2.3	2.49	2.49	2.49
5.8	0.7627	5.8	0.6429	5.8	1	2.4	2.4083	2.4083	2.4083
5.6	0.7627	5.6	0.6429	5.6	1	2.5	2.3664	2.3664	2.3664
5.6	0.7627	5.6	0.6429	5.6	1	2.6	2.3664	2.3664	2.3664
5.4	0.7627	5.4	0.6429	5.4	1	2.7	2.3238	2.3238	2.3238
5.6	0.7627	5.6	0.6429	5.6	1	2.8	2.3664	2.3664	2.3664
5.4	0.7627	5.4	0.6429	5.4	1	2.9	2.3238	2.3238	2.3238
5.2	0.7627	5.2	0.6429	5.2	1	3	2.2804	2.2804	2.2804
5	0.7627	5	0.6429	5	1	3.1	2.2361	2.2361	2.2361
4.8	0.8163	4.8	0.6429	4.8	1	3.2	2.1909	2.1909	2.1909
5.2	0.7627	5.2	0.6429	5.2	1	3.3	2.2804	2.2804	2.2804
5	0.7627	5	0.6429	5	1	3.4	2.2361	2.2361	2.2361
4.8	0.7627	4.8	0.6429	4.8	1	3.5	2.1909	2.1909	2.1909
4.6	0.8163	4.6	0.6429	4.6	1	3.6	2.1448	2.1448	2.1448
6	0.7813	6	0.6429	6	1	3.7	2.4495	2.4495	2.4495
5.6	0.7813	5.6	0.6429	5.6	1	3.8	2.3664	2.3664	2.3664
5.4	0.7813	5.4	0.6429	5.4	1	3.9	2.3238	2.3238	2.3238
5.4	0.7813	5.4	0.6429	5.4	1	4	2.3238	2.3238	2.3238
5.2	0.7813	5.2	0.6429	5.2	1	4.1	2.2804	2.2804	2.2804
5	0.7813	5	0.6429	5	1	4.2	2.2361	2.2361	2.2361
4.8	0.7813	4.8	0.6429	4.8	1	0.1	2.1909	2.1909	2.1909
5	0.7813	5	0.6429	5	1	0.2	2.2361	2.2361	2.2361
4.8	0.7813	4.8	0.6429	4.8	1	0.3	2.1909	2.1909	2.1909
4.6	0.7813	4.6	0.6429	4.6	1	0.4	2.1448	2.1448	2.1448
4.4	0.8163	4.4	0.6429	4.4	1	0.5	2.0976	2.0976	2.0976
4.8	0.7813	4.8	0.6429	4.8	1	0.6	2.1909	2.1909	2.1909
4.4	0.7813	4.4	0.6429	4.4	1	0.7	2.0976	2.0976	2.0976
4.2	0.8163	4.2	0.6429	4.2	1	0.8	2.0494	2.0494	2.0494
4.2	0.7813	4.2	0.6429	4.2	1	0.9	2.0494	2.0494	2.0494
4	0.8163	4	0.6429	4	1	1	2	2	2
8.6	0.7223	8.6	0.6429	8.6	1	1.1	2.9326	2.9326	2.9326
8.4	0.7223	8.4	0.6429	8.4	1	1.2	2.8983	2.8983	2.8983
8	0.7223	8	0.6429	8	1	1.3	2.8284	2.8284	2.8284
7.6	0.7223	7.6	0.6429	7.6	1	1.4	2.7568	2.7568	2.7568
7.4	0.7223	7.4	0.6429	7.4	1	1.5	2.7203	2.7203	2.7203
7.8	0.7282	7.8	0.6429	7.8	1	1.6	2.7928	2.7928	2.7928
7.2	0.7282	7.2	0.6429	7.2	1	1.7	2.6833	2.6833	2.6833
7	0.7282	7	0.6429	7	1	1.8	2.6458	2.6458	2.6458
6.8	0.7282	6.8	0.6429	6.8	1	1.9	2.6077	2.6077	2.6077
6.6	0.7589	6.6	0.6429	6.6	1	2	2.569	2.569	2.569
6.8	0.7282	6.8	0.6429	6.8	1	2.1	2.6077	2.6077	2.6077
6.6	0.7282	6.6	0.6429	6.6	1	2.2	2.569	2.569	2.569
6.4	0.7282	6.4	0.6429	6.4	1	2.3	2.5298	2.5298	2.5298
6.2	0.7589	6.2	0.6429	6.2	1	2.4	2.49	2.49	2.49
6.2	0.7282	6.2	0.6429	6.2	1	2.5	2.49	2.49	2.49
6	0.7589	6	0.6429	6	1	2.6	2.4495	2.4495	2.4495
7.6	0.7357	7.6	0.6429	7.6	1	2.7	2.7568	2.7568	2.7568
7	0.7357	7	0.6429	7	1	2.8	2.6458	2.6458	2.6458
6.8	0.7357	6.8	0.6429	6.8	1	2.9	2.6077	2.6077	2.6077
6.6	0.7357	6.6	0.6429	6.6	1	3	2.569	2.569	2.569
6.4	0.7589	6.4	0.6429	6.4	1	3.1	2.5298	2.5298	2.5298
6.8	0.745	6.8	0.6429	6.8	1	3.2	2.6077	2.6077	2.6077
6.4	0.745	6.4	0.6429	6.4	1	3.3	2.5298	2.5298	2.5298
6.2	0.745	6.2	0.6429	6.2	1	3.4	2.49	2.49	2.49
6	0.745	6	0.6429	6	1	3.5	2.4495	2.4495	2.4495
5.8	0.7589	5.8	0.6429	5.8	1	3.6	2.4083	2.4083	2.4083
6.2	0.745	6.2	0.6429	6.2	1	3.7	2.49	2.49	2.49
5.8	0.745	5.8	0.6429	5.8	1	3.8	2.4083	2.4083	2.4083
5.6	0.7589	5.6	0.6429	5.6	1	3.9	2.3664	2.3664	2.3664
5.6	0.745	5.6	0.6429	5.6	1	4	2.3664	2.3664	2.3664
5.4	0.7589	5.4	0.6429	5.4	1	4.1	2.3238	2.3238	2.3238
5.2	0.7589	5.2	0.6429	5.2	1	4.2	2.2804	2.2804	2.2804
6.2	0.7627	6.2	0.6429	6.2	1	0.1	2.49	2.49	2.49
6	0.7627	6	0.6429	6	1	0.2	2.4495	2.4495	2.4495
6	0.7627	6	0.6429	6	1	0.3	2.4495	2.4495	2.4495
5.6	0.7627	5.6	0.6429	5.6	1	0.4	2.3664	2.3664	2.3664
5.4	0.7627	5.4	0.6429	5.4	1	0.5	2.3238	2.3238	2.3238
5.4	0.7627	5.4	0.6429	5.4	1	0.6	2.3238	2.3238	2.3238
5.2	0.7627	5.2	0.6429	5.2	1	0.7	2.2804	2.2804	2.2804
5.4	0.7627	5.4	0.6429	5.4	1	0.8	2.3238	2.3238	2.3238
5.2	0.7627	5.2	0.6429	5.2	1	0.9	2.2804	2.2804	2.2804
5	0.7627	5	0.6429	5	1	1	2.2361	2.2361	2.2361
4.8	0.7627	4.8	0.6429	4.8	1	1.1	2.1909	2.1909	2.1909
4.6	0.8163	4.6	0.6429	4.6	1	1.2	2.1448	2.1448	2.1448
5	0.7627	5	0.6429	5	1	1.3	2.2361	2.2361	2.2361
4.8	0.7627	4.8	0.6429	4.8	1	1.4	2.1909	2.1909	2.1909
4.6	0.7627	4.6	0.6429	4.6	1	1.5	2.1448	2.1448	2.1448
4.4	0.8163	4.4	0.6429	4.4	1	1.6	2.0976	2.0976	2.0976
7.4	0.7529	7.4	0.6429	7.4	1	1.7	2.7203	2.7203	2.7203
6.6	0.7529	6.6	0.6429	6.6	1	1.8	2.569	2.569	2.569
6.2	0.7529	6.2	0.6429	6.2	1	1.9	2.49	2.49	2.49
6	0.7529	6	0.6429	6	1	2	2.4495	2.4495	2.4495
5.8	0.7529	5.8	0.6429	5.8	1	2.1	2.4083	2.4083	2.4083
5.6	0.7589	5.6	0.6429	5.6	1	2.2	2.3664	2.3664	2.3664
6	0.7627	6	0.6429	6	1	2.3	2.4495	2.4495	2.4495
5.8	0.7627	5.8	0.6429	5.8	1	2.4	2.4083	2.4083	2.4083
5.8	0.7627	5.8	0.6429	5.8	1	2.5	2.4083	2.4083	2.4083
5.4	0.7627	5.4	0.6429	5.4	1	2.6	2.3238	2.3238	2.3238
5.2	0.7627	5.2	0.6429	5.2	1	2.7	2.2804	2.2804	2.2804
5.2	0.7627	5.2	0.6429	5.2	1	2.8	2.2804	2.2804	2.2804
5	0.7627	5	0.6429	5	1	2.9	2.2361	2.2361	2.2361
5.2	0.7627	5.2	0.6429	5.2	1	3	2.2804	2.2804	2.2804
5	0.7627	5	0.6429	5	1	3.1	2.2361	2.2361	2.2361
4.8	0.7627	4.8	0.6429	4.8	1	3.2	2.1909	2.1909	2.1909
4.6	0.7627	4.6	0.6429	4.6	1	3.3	2.1448	2.1448	2.1448
4.4	0.8163	4.4	0.6429	4.4	1	3.4	2.0976	2.0976	2.0976
5.6	0.7813	5.6	0.6429	5.6	1	3.5	2.3664	2.3664	2.3664
5.2	0.7813	5.2	0.6429	5.2	1	3.6	2.2804	2.2804	2.2804
5	0.7813	5	0.6429	5	1	3.7	2.2361	2.2361	2.2361
5	0.7813	5	0.6429	5	1	3.8	2.2361	2.2361	2.2361
4.8	0.7813	4.8	0.6429	4.8	1	3.9	2.1909	2.1909	2.1909
4.6	0.7813	4.6	0.6429	4.6	1	4	2.1448	2.1448	2.1448
4.4	0.7813	4.4	0.6429	4.4	1	4.1	2.0976	2.0976	2.0976
4.6	0.7813	4.6	0.6429	4.6	1	4.2	2.1448	2.1448	2.1448
4.4	0.7813	4.4	0.6429	4.4	1	0.1	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	0.2	2.0494	2.0494	2.0494
4	0.8163	4	0.6429	4	1	0.3	2	2	2
4.4	0.7813	4.4	0.6429	4.4	1	0.4	2.0976	2.0976	2.0976
4	0.7813	4	0.6429	4	1	0.5	2	2	2
3.8	0.8163	3.8	0.6429	3.8	1	0.6	1.9494	1.9494	1.9494
5.4	0.7813	5.4	0.6429	5.4	1	0.7	2.3238	2.3238	2.3238
4.8	0.7813	4.8	0.6429	4.8	1	0.8	2.1909	2.1909	2.1909
4.6	0.7813	4.6	0.6429	4.6	1	0.9	2.1448	2.1448	2.1448
4.4	0.7813	4.4	0.6429	4.4	1	1	2.0976	2.0976	2.0976
4.4	0.7813	4.4	0.6429	4.4	1	1.1	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	1.2	2.0494	2.0494	2.0494
4	0.7813	4	0.6429	4	1	1.3	2	2	2
3.8	0.8163	3.8	0.6429	3.8	1	1.4	1.9494	1.9494	1.9494
4.2	0.7813	4.2	0.6429	4.2	1	1.5	2.0494	2.0494	2.0494
3.8	0.7813	3.8	0.6429	3.8	1	1.6	1.9494	1.9494	1.9494
3.6	0.8163	3.6	0.6429	3.6	1	1.7	1.8974	1.8974	1.8974
3.6	0.7813	3.6	0.6429	3.6	1	1.8	1.8974	1.8974	1.8974
3.4	0.8163	3.4	0.6429	3.4	1	1.9	1.8439	1.8439	1.8439
3.2	0.8163	3.2	0.6429	3.2	1	2	1.7889	1.7889	1.7889
6.4	0.771	6.4	0.6429	6.4	1	2.1	2.5298	2.5298	2.5298
5.8	0.771	5.8	0.6429	5.8	1	2.2	2.4083	2.4083	2.4083
5.6	0.771	5.6	0.6429	5.6	1	2.3	2.3664	2.3664	2.3664
5.6	0.771	5.6	0.6429	5.6	1	2.4	2.3664	2.3664	2.3664
5.2	0.771	5.2	0.6429	5.2	1	2.5	2.2804	2.2804	2.2804
5	0.771	5	0.6429	5	1	2.6	2.2361	2.2361	2.2361
5	0.771	5	0.6429	5	1	2.7	2.2361	2.2361	2.2361
4.8	0.771	4.8	0.6429	4.8	1	2.8	2.1909	2.1909	2.1909
5.4	0.7813	5.4	0.6429	5.4	1	2.9	2.3238	2.3238	2.3238
5	0.7813	5	0.6429	5	1	3	2.2361	2.2361	2.2361
4.8	0.7813	4.8	0.6429	4.8	1	3.1	2.1909	2.1909	2.1909
4.8	0.7813	4.8	0.6429	4.8	1	3.2	2.1909	2.1909	2.1909
4.6	0.7813	4.6	0.6429	4.6	1	3.3	2.1448	2.1448	2.1448
4.4	0.7813	4.4	0.6429	4.4	1	3.4	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	3.5	2.0494	2.0494	2.0494
4.4	0.7813	4.4	0.6429	4.4	1	3.6	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	3.7	2.0494	2.0494	2.0494
4	0.7813	4	0.6429	4	1	3.8	2	2	2
3.8	0.8163	3.8	0.6429	3.8	1	3.9	1.9494	1.9494	1.9494
5.2	0.7813	5.2	0.6429	5.2	1	4	2.2804	2.2804	2.2804
4.6	0.7813	4.6	0.6429	4.6	1	4.1	2.1448	2.1448	2.1448
4.4	0.7813	4.4	0.6429	4.4	1	4.2	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	0.1	2.0494	2.0494	2.0494
4.2	0.7813	4.2	0.6429	4.2	1	0.2	2.0494	2.0494	2.0494
4	0.7813	4	0.6429	4	1	0.3	2	2	2
3.8	0.7813	3.8	0.6429	3.8	1	0.4	1.9494	1.9494	1.9494
3.6	0.8163	3.6	0.6429	3.6	1	0.5	1.8974	1.8974	1.8974
4	0.7813	4	0.6429	4	1	0.6	2	2	2
3.6	0.7813	3.6	0.6429	3.6	1	0.7	1.8974	1.8974	1.8974
3.4	0.8163	3.4	0.6429	3.4	1	0.8	1.8439	1.8439	1.8439
3.4	0.7813	3.4	0.6429	3.4	1	0.9	1.8439	1.8439	1.8439
3.2	0.8163	3.2	0.6429	3.2	1	1	1.7889	1.7889	1.7889
4.4	0.7813	4.4	0.6429	4.4	1	1.1	2.0976	2.0976	2.0976
4	0.7813	4	0.6429	4	1	1.2	2	2	2
3.8	0.7813	3.8	0.6429	3.8	1	1.3	1.9494	1.9494	1.9494
3.6	0.7813	3.6	0.6429	3.6	1	1.4	1.8974	1.8974	1.8974
3.8	0.7813	3.8	0.6429	3.8	1	1.5	1.9494	1.9494	1.9494
3.4	0.7813	3.4	0.6429	3.4	1	1.6	1.8439	1.8439	1.8439
3.2	0.8163	3.2	0.6429	3.2	1	1.7	1.7889	1.7889	1.7889
3.2	0.7813	3.2	0.6429	3.2	1	1.8	1.7889	1.7889	1.7889
3	0.8163	3	0.6429	3	1	1.9	1.7321	1.7321	1.7321
2.8	0.8163	2.8	0.6429	2.8	1	2	1.6733	1.6733	1.6733
2.6	0.8929	2.6	0.6429	2.6	1	2.1	1.6125	1.6125	1.6125
3.8	0.7813	3.8	0.6429	3.8	1	2.2	1.9494	1.9494	1.9494
3.6	0.7813	3.6	0.6429	3.6	1	2.3	1.8974	1.8974	1.8974
3.6	0.7813	3.6	0.6429	3.6	1	2.4	1.8974	1.8974	1.8974
3.2	0.7813	3.2	0.6429	3.2	1	2.5	1.7889	1.7889	1.7889
3	0.8163	3	0.6429	3	1	2.6	1.7321	1.7321	1.7321
3	0.7813	3	0.6429	3	1	2.7	1.7321	1.7321	1.7321
2.8	0.8163	2.8	0.6429	2.8	1	2.8	1.6733	1.6733	1.6733
2.6	0.8163	2.6	0.6429	2.6	1	2.9	1.6125	1.6125	1.6125
2.4	0.8929	2.4	0.6429	2.4	1	3	1.5492	1.5492	1.5492
7.8	0.7389	7.8	0.6429	7.8	1	3.1	2.7928	2.7928	2.7928
7.4	0.7389	7.4	0.6429	7.4	1	3.2	2.7203	2.7203	2.7203
7.2	0.7389	7.2	0.6429	7.2	1	3.3	2.6833	2.6833	2.6833
7.4	0.7389	7.4	0.6429	7.4	1	3.4	2.7203	2.7203	2.7203
6.8	0.7389	6.8	0.6429	6.8	1	3.5	2.6077	2.6077	2.6077
6.6	0.7389	6.6	0.6429	6.6	1	3.6	2.569	2.569	2.569
6.4	0.7389	6.4	0.6429	6.4	1	3.7	2.5298	2.5298	2.5298
6.2	0.7589	6.2	0.6429	6.2	1	3.8	2.49	2.49	2.49
6.6	0.745	6.6	0.6429	6.6	1	3.9	2.569	2.569	2.569
6.2	0.745	6.2	0.6429	6.2	1	4	2.49	2.49	2.49
6	0.745	6	0.6429	6	1	4.1	2.4495	2.4495	2.4495
5.8	0.745	5.8	0.6429	5.8	1	4.2	2.4083	2.4083	2.4083
5.6	0.7589	5.6	0.6429	5.6	1	0.1	2.3664	2.3664	2.3664
6	0.745	6	0.6429	6	1	0.2	2.4495	2.4495	2.4495
5.6	0.745	5.6	0.6429	5.6	1	0.3	2.3664	2.3664	2.3664
5.4	0.7589	5.4	0.6429	5.4	1	0.4	2.3238	2.3238	2.3238
5.4	0.745	5.4	0.6429	5.4	1	0.5	2.3238	2.3238	2.3238
5.2	0.7589	5.2	0.6429	5.2	1	0.6	2.2804	2.2804	2.2804
5	0.7589	5	0.6429	5	1	0.7	2.2361	2.2361	2.2361
7.2	0.7529	7.2	0.6429	7.2	1	0.8	2.6833	2.6833	2.6833
6.4	0.7529	6.4	0.6429	6.4	1	0.9	2.5298	2.5298	2.5298
6	0.7529	6	0.6429	6	1	1	2.4495	2.4495	2.4495
5.8	0.7529	5.8	0.6429	5.8	1	1.1	2.4083	2.4083	2.4083
5.6	0.7529	5.6	0.6429	5.6	1	1.2	2.3664	2.3664	2.3664
5.4	0.7589	5.4	0.6429	5.4	1	1.3	2.3238	2.3238	2.3238
5.8	0.7627	5.8	0.6429	5.8	1	1.4	2.4083	2.4083	2.4083
5.6	0.7627	5.6	0.6429	5.6	1	1.5	2.3664	2.3664	2.3664
5.6	0.7627	5.6	0.6429	5.6	1	1.6	2.3664	2.3664	2.3664
5.2	0.7627	5.2	0.6429	5.2	1	1.7	2.2804	2.2804	2.2804
5	0.7627	5	0.6429	5	1	1.8	2.2361	2.2361	2.2361
5	0.7627	5	0.6429	5	1	1.9	2.2361	2.2361	2.2361
4.8	0.7627	4.8	0.6429	4.8	1	2	2.1909	2.1909	2.1909
5	0.7627	5	0.6429	5	1	2.1	2.2361	2.2361	2.2361
4.8	0.7627	4.8	0.6429	4.8	1	2.2	2.1909	2.1909	2.1909
4.6	0.7627	4.6	0.6429	4.6	1	2.3	2.1448	2.1448	2.1448
4.4	0.7627	4.4	0.6429	4.4	1	2.4	2.0976	2.0976	2.0976
4.2	0.8163	4.2	0.6429	4.2	1	2.5	2.0494	2.0494	2.0494
5.4	0.7813	5.4	0.6429	5.4	1	2.6	2.3238	2.3238	2.3238
5	0.7813	5	0.6429	5	1	2.7	2.2361	2.2361	2.2361
4.8	0.7813	4.8	0.6429	4.8	1	2.8	2.1909	2.1909	2.1909
4.8	0.7813	4.8	0.6429	4.8	1	2.9	2.1909	2.1909	2.1909
4.6	0.7813	4.6	0.6429	4.6	1	3	2.1448	2.1448	2.1448
4.4	0.7813	4.4	0.6429	4.4	1	3.1	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	3.2	2.0494	2.0494	2.0494
4.4	0.7813	4.4	0.6429	4.4	1	3.3	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	3.4	2.0494	2.0494	2.0494
4	0.7813	4	0.6429	4	1	3.5	2	2	2
3.8	0.8163	3.8	0.6429	3.8	1	3.6	1.9494	1.9494	1.9494
4.2	0.7813	4.2	0.6429	4.2	1	3.7	2.0494	2.0494	2.0494
3.8	0.7813	3.8	0.6429	3.8	1	3.8	1.9494	1.9494	1.9494
3.6	0.8163	3.6	0.6429	3.6	1	3.9	1.8974	1.8974	1.8974
6.2	0.771	6.2	0.6429	6.2	1	4	2.49	2.49	2.49
5.6	0.771	5.6	0.6429	5.6	1	4.1	2.3664	2.3664	2.3664
5.4	0.771	5.4	0.6429	5.4	1	4.2	2.3238	2.3238	2.3238
5.4	0.771	5.4	0.6429	5.4	1	0.1	2.3238	2.3238	2.3238
5	0.771	5	0.6429	5	1	0.2	2.2361	2.2361	2.2361
4.8	0.771	4.8	0.6429	4.8	1	0.3	2.1909	2.1909	2.1909
4.8	0.771	4.8	0.6429	4.8	1	0.4	2.1909	2.1909	2.1909
4.6	0.771	4.6	0.6429	4.6	1	0.5	2.1448	2.1448	2.1448
5.2	0.7813	5.2	0.6429	5.2	1	0.6	2.2804	2.2804	2.2804
4.8	0.7813	4.8	0.6429	4.8	1	0.7	2.1909	2.1909	2.1909
4.6	0.7813	4.6	0.6429	4.6	1	0.8	2.1448	2.1448	2.1448
4.6	0.7813	4.6	0.6429	4.6	1	0.9	2.1448	2.1448	2.1448
4.4	0.7813	4.4	0.6429	4.4	1	1	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	1.1	2.0494	2.0494	2.0494
4	0.7813	4	0.6429	4	1	1.2	2	2	2
4.2	0.7813	4.2	0.6429	4.2	1	1.3	2.0494	2.0494	2.0494
4	0.7813	4	0.6429	4	1	1.4	2	2	2
3.8	0.7813	3.8	0.6429	3.8	1	1.5	1.9494	1.9494	1.9494
3.6	0.8163	3.6	0.6429	3.6	1	1.6	1.8974	1.8974	1.8974
5	0.7813	5	0.6429	5	1	1.7	2.2361	2.2361	2.2361
4.4	0.7813	4.4	0.6429	4.4	1	1.8	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	1.9	2.0494	2.0494	2.0494
4	0.7813	4	0.6429	4	1	2	2	2	2
4	0.7813	4	0.6429	4	1	2.1	2	2	2
3.8	0.7813	3.8	0.6429	3.8	1	2.2	1.9494	1.9494	1.9494
3.6	0.7813	3.6	0.6429	3.6	1	2.3	1.8974	1.8974	1.8974
3.4	0.8163	3.4	0.6429	3.4	1	2.4	1.8439	1.8439	1.8439
3.8	0.7813	3.8	0.6429	3.8	1	2.5	1.9494	1.9494	1.9494
3.4	0.7813	3.4	0.6429	3.4	1	2.6	1.8439	1.8439	1.8439
3.2	0.8163	3.2	0.6429	3.2	1	2.7	1.7889	1.7889	1.7889
3.2	0.7813	3.2	0.6429	3.2	1	2.8	1.7889	1.7889	1.7889
3	0.8163	3	0.6429	3	1	2.9	1.7321	1.7321	1.7321
4.2	0.7813	4.2	0.6429	4.2	1	3	2.0494	2.0494	2.0494
3.8	0.7813	3.8	0.6429	3.8	1	3.1	1.9494	1.9494	1.9494
3.6	0.7813	3.6	0.6429	3.6	1	3.2	1.8974	1.8974	1.8974
3.4	0.7813	3.4	0.6429	3.4	1	3.3	1.8439	1.8439	1.8439
3.6	0.7813	3.6	0.6429	3.6	1	3.4	1.8974	1.8974	1.8974
3.2	0.7813	3.2	0.6429	3.2	1	3.5	1.7889	1.7889	1.7889
3	0.8163	3	0.6429	3	1	3.6	1.7321	1.7321	1.7321
3	0.7813	3	0.6429	3	1	3.7	1.7321	1.7321	1.7321
2.8	0.8163	2.8	0.6429	2.8	1	3.8	1.6733	1.6733	1.6733
2.6	0.8163	2.6	0.6429	2.6	1	3.9	1.6125	1.6125	1.6125
2.4	0.8929	2.4	0.6429	2.4	1	4	1.5492	1.5492	1.5492
5.4	0.7899	5.4	0.6429	5.4	1	4.1	2.3238	2.3238	2.3238
5.2	0.7899	5.2	0.6429	5.2	1	4.2	2.2804	2.2804	2.2804
5	0.7899	5	0.6429	5	1	0.1	2.2361	2.2361	2.2361
4.6	0.7899	4.6	0.6429	4.6	1	0.2	2.1448	2.1448	2.1448
4.4	0.7899	4.4	0.6429	4.4	1	0.3	2.0976	2.0976	2.0976
4.4	0.7899	4.4	0.6429	4.4	1	0.4	2.0976	2.0976	2.0976
4.2	0.7899	4.2	0.6429	4.2	1	0.5	2.0494	2.0494	2.0494
4	0.7899	4	0.6429	4	1	0.6	2	2	2
3.8	0.7899	3.8	0.6429	3.8	1	0.7	1.9494	1.9494	1.9494
4.8	0.7899	4.8	0.6429	4.8	1	0.8	2.1909	2.1909	2.1909
4.2	0.7899	4.2	0.6429	4.2	1	0.9	2.0494	2.0494	2.0494
4	0.7899	4	0.6429	4	1	1	2	2	2
3.8	0.7899	3.8	0.6429	3.8	1	1.1	1.9494	1.9494	1.9494
3.8	0.7899	3.8	0.6429	3.8	1	1.2	1.9494	1.9494	1.9494
3.6	0.7899	3.6	0.6429	3.6	1	1.3	1.8974	1.8974	1.8974
3.4	0.7899	3.4	0.6429	3.4	1	1.4	1.8439	1.8439	1.8439
3.2	0.8163	3.2	0.6429	3.2	1	1.5	1.7889	1.7889	1.7889
3.6	0.7899	3.6	0.6429	3.6	1	1.6	1.8974	1.8974	1.8974
3.2	0.7899	3.2	0.6429	3.2	1	1.7	1.7889	1.7889	1.7889
3	0.8163	3	0.6429	3	1	1.8	1.7321	1.7321	1.7321
4	0.7899	4	0.6429	4	1	1.9	2	2	2
3.6	0.7899	3.6	0.6429	3.6	1	2	1.8974	1.8974	1.8974
3.4	0.7899	3.4	0.6429	3.4	1	2.1	1.8439	1.8439	1.8439
3.2	0.7899	3.2	0.6429	3.2	1	2.2	1.7889	1.7889	1.7889
3.4	0.7899	3.4	0.6429	3.4	1	2.3	1.8439	1.8439	1.8439
3	0.7899	3	0.6429	3	1	2.4	1.7321	1.7321	1.7321
2.8	0.8163	2.8	0.6429	2.8	1	2.5	1.6733	1.6733	1.6733
2.8	0.7899	2.8	0.6429	2.8	1	2.6	1.6733	1.6733	1.6733
2.6	0.8163	2.6	0.6429	2.6	1	2.7	1.6125	1.6125	1.6125
2.4	0.8163	2.4	0.6429	2.4	1	2.8	1.5492	1.5492	1.5492
3.4	0.7899	3.4	0.6429	3.4	1	2.9	1.8439	1.8439	1.8439
3.2	0.7899	3.2	0.6429	3.2	1	3	1.7889	1.7889	1.7889
3.2	0.7899	3.2	0.6429	3.2	1	3.1	1.7889	1.7889	1.7889
2.8	0.7899	2.8	0.6429	2.8	1	3.2	1.6733	1.6733	1.6733
2.6	0.8163	2.6	0.6429	2.6	1	3.3	1.6125	1.6125	1.6125
2.6	0.7899	2.6	0.6429	2.6	1	3.4	1.6125	1.6125	1.6125
2.4	0.8163	2.4	0.6429	2.4	1	3.5	1.5492	1.5492	1.5492
2.2	0.8163	2.2	0.6429	2.2	1	3.6	1.4832	1.4832	1.4832
2	0.8929	2	0.6429	2	1	3.7	1.4142	1.4142	1.4142
3	0.7899	3	0.6429	3	1	3.8	1.7321	1.7321	1.7321
2.6	0.7899	2.6	0.6429	2.6	1	3.9	1.6125	1.6125	1.6125
2.4	0.7899	2.4	0.6429	2.4	1	4	1.5492	1.5492	1.5492
2.2	0.8163	2.2	0.6429	2.2	1	4.1	1.4832	1.4832	1.4832
2	0.8163	2	0.6429	2	1	4.2	1.4142	1.4142	1.4142
1.8	0.8929	1.8	0.6429	1.8	1	0.1	1.3416	1.3416	1.3416
4.8	0.8098	4.8	0.6429	4.8	1	0.2	2.1909	2.1909	2.1909
4.4	0.8098	4.4	0.6429	4.4	1	0.3	2.0976	2.0976	2.0976
4.2	0.8098	4.2	0.6429	4.2	1	0.4	2.0494	2.0494	2.0494
4.6	0.8098	4.6	0.6429	4.6	1	0.5	2.1448	2.1448	2.1448
4	0.8098	4	0.6429	4	1	0.6	2	2	2
3.8	0.8098	3.8	0.6429	3.8	1	0.7	1.9494	1.9494	1.9494
3.6	0.8098	3.6	0.6429	3.6	1	0.8	1.8974	1.8974	1.8974
3.6	0.8098	3.6	0.6429	3.6	1	0.9	1.8974	1.8974	1.8974
3.4	0.8098	3.4	0.6429	3.4	1	1	1.8439	1.8439	1.8439
3.2	0.8098	3.2	0.6429	3.2	1	1.1	1.7889	1.7889	1.7889
3	0.8163	3	0.6429	3	1	1.2	1.7321	1.7321	1.7321
3.8	0.8098	3.8	0.6429	3.8	1	1.3	1.9494	1.9494	1.9494
3.4	0.8098	3.4	0.6429	3.4	1	1.4	1.8439	1.8439	1.8439
3.2	0.8098	3.2	0.6429	3.2	1	1.5	1.7889	1.7889	1.7889
3	0.8098	3	0.6429	3	1	1.6	1.7321	1.7321	1.7321
3.2	0.8098	3.2	0.6429	3.2	1	1.7	1.7889	1.7889	1.7889
2.8	0.8098	2.8	0.6429	2.8	1	1.8	1.6733	1.6733	1.6733
2.6	0.8163	2.6	0.6429	2.6	1	1.9	1.6125	1.6125	1.6125
2.6	0.8098	2.6	0.6429	2.6	1	2	1.6125	1.6125	1.6125
2.4	0.8163	2.4	0.6429	2.4	1	2.1	1.5492	1.5492	1.5492
3.2	0.8098	3.2	0.6429	3.2	1	2.2	1.7889	1.7889	1.7889
3	0.8098	3	0.6429	3	1	2.3	1.7321	1.7321	1.7321
3	0.8098	3	0.6429	3	1	2.4	1.7321	1.7321	1.7321
2.6	0.8098	2.6	0.6429	2.6	1	2.5	1.6125	1.6125	1.6125
2.4	0.8163	2.4	0.6429	2.4	1	2.6	1.5492	1.5492	1.5492
2.4	0.8098	2.4	0.6429	2.4	1	2.7	1.5492	1.5492	1.5492
2.2	0.8163	2.2	0.6429	2.2	1	2.8	1.4832	1.4832	1.4832
2	0.8163	2	0.6429	2	1	2.9	1.4142	1.4142	1.4142
1.8	0.8929	1.8	0.6429	1.8	1	3	1.3416	1.3416	1.3416
2.8	0.8098	2.8	0.6429	2.8	1	3.1	1.6733	1.6733	1.6733
2.4	0.8098	2.4	0.6429	2.4	1	3.2	1.5492	1.5492	1.5492
2.2	0.8098	2.2	0.6429	2.2	1	3.3	1.4832	1.4832	1.4832
2	0.8163	2	0.6429	2	1	3.4	1.4142	1.4142	1.4142
1.8	0.8163	1.8	0.6429	1.8	1	3.5	1.3416	1.3416	1.3416
1.6	0.8929	1.6	0.6429	1.6	1	3.6	1.2649	1.2649	1.2649
2.6	0.8098	2.6	0.6429	2.6	1	3.7	1.6125	1.6125	1.6125
2	0.8098	2	0.6429	2	1	3.8	1.4142	1.4142	1.4142
1.8	0.8163	1.8	0.6429	1.8	1	3.9	1.3416	1.3416	1.3416
1.6	0.8163	1.6	0.6429	1.6	1	4	1.2649	1.2649	1.2649
1.4	0.8929	1.4	0.6429	1.4	1	4.1	1.1832	1.1832	1.1832
1.8	0.8098	1.8	0.6429	1.8	1	4.2	1.3416	1.3416	1.3416
1.4	0.8163	1.4	0.6429	1.4	1	0.1	1.1832	1.1832	1.1832
1.2	0.8929	1.2	0.6429	1.2	1	0.2	1.0954	1.0954	1.0954
7.2	0.7563	7.2	0.6429	7.2	1	0.3	2.6833	2.6833	2.6833
6.6	0.7563	6.6	0.6429	6.6	1	0.4	2.569	2.569	2.569
6.4	0.7563	6.4	0.6429	6.4	1	0.5	2.5298	2.5298	2.5298
6.2	0.7563	6.2	0.6429	6.2	1	0.6	2.49	2.49	2.49
6	0.7589	6	0.6429	6	1	0.7	2.4495	2.4495	2.4495
7	0.7563	7	0.6429	7	1	0.8	2.6458	2.6458	2.6458
6.2	0.7563	6.2	0.6429	6.2	1	0.9	2.49	2.49	2.49
5.8	0.7563	5.8	0.6429	5.8	1	1	2.4083	2.4083	2.4083
5.6	0.7563	5.6	0.6429	5.6	1	1.1	2.3664	2.3664	2.3664
5.4	0.7563	5.4	0.6429	5.4	1	1.2	2.3238	2.3238	2.3238
5.2	0.7589	5.2	0.6429	5.2	1	1.3	2.2804	2.2804	2.2804
5.6	0.7627	5.6	0.6429	5.6	1	1.4	2.3664	2.3664	2.3664
5.4	0.7627	5.4	0.6429	5.4	1	1.5	2.3238	2.3238	2.3238
5.4	0.7627	5.4	0.6429	5.4	1	1.6	2.3238	2.3238	2.3238
5	0.7627	5	0.6429	5	1	1.7	2.2361	2.2361	2.2361
4.8	0.7627	4.8	0.6429	4.8	1	1.8	2.1909	2.1909	2.1909
4.8	0.7627	4.8	0.6429	4.8	1	1.9	2.1909	2.1909	2.1909
4.6	0.7627	4.6	0.6429	4.6	1	2	2.1448	2.1448	2.1448
4.8	0.7627	4.8	0.6429	4.8	1	2.1	2.1909	2.1909	2.1909
4.6	0.7627	4.6	0.6429	4.6	1	2.2	2.1448	2.1448	2.1448
4.4	0.7627	4.4	0.6429	4.4	1	2.3	2.0976	2.0976	2.0976
4.2	0.7627	4.2	0.6429	4.2	1	2.4	2.0494	2.0494	2.0494
4	0.8163	4	0.6429	4	1	2.5	2	2	2
6	0.771	6	0.6429	6	1	2.6	2.4495	2.4495	2.4495
5.4	0.771	5.4	0.6429	5.4	1	2.7	2.3238	2.3238	2.3238
5.2	0.771	5.2	0.6429	5.2	1	2.8	2.2804	2.2804	2.2804
5.2	0.771	5.2	0.6429	5.2	1	2.9	2.2804	2.2804	2.2804
4.8	0.771	4.8	0.6429	4.8	1	3	2.1909	2.1909	2.1909
4.6	0.771	4.6	0.6429	4.6	1	3.1	2.1448	2.1448	2.1448
4.6	0.771	4.6	0.6429	4.6	1	3.2	2.1448	2.1448	2.1448
4.4	0.771	4.4	0.6429	4.4	1	3.3	2.0976	2.0976	2.0976
5	0.7813	5	0.6429	5	1	3.4	2.2361	2.2361	2.2361
4.6	0.7813	4.6	0.6429	4.6	1	3.5	2.1448	2.1448	2.1448
4.4	0.7813	4.4	0.6429	4.4	1	3.6	2.0976	2.0976	2.0976
4.4	0.7813	4.4	0.6429	4.4	1	3.7	2.0976	2.0976	2.0976
4.2	0.7813	4.2	0.6429	4.2	1	3.8	2.0494	2.0494	2.0494
4	0.7813	4	0.6429	4	1	3.9	2	2	2
3.8	0.7813	3.8	0.6429	3.8	1	4	1.9494	1.9494	1.9494
4	0.7813	4	0.6429	4	1	4.1	2	2	2
3.8	0.7813	3.8	0.6429	3.8	1	4.2	1.9494	1.9494	1.9494
3.6	0.7813	3.6	0.6429	3.6	1	0.1	1.8974	1.8974	1.8974
3.4	0.8163	3.4	0.6429	3.4	1	0.2	1.8439	1.8439	1.8439
4.8	0.7813	4.8	0.6429	4.8	1	0.3	2.1909	2.1909	2.1909
4.2	0.7813	4.2	0.6429	4.2	1	0.4	2.0494	2.0494	2.0494
4	0.7813	4	0.6429	4	1	0.5	2	2	2
3.8	0.7813	3.8	0.6429	3.8	1	0.6	1.9494	1.9494	1.9494
3.8	0.7813	3.8	0.6429	3.8	1	0.7	1.9494	1.9494	1.9494
3.6	0.7813	3.6	0.6429	3.6	1	0.8	1.8974	1.8974	1.8974
3.4	0.7813	3.4	0.6429	3.4	1	0.9	1.8439	1.8439	1.8439
3.2	0.8163	3.2	0.6429	3.2	1	1	1.7889	1.7889	1.7889
3.6	0.7813	3.6	0.6429	3.6	1	1.1	1.8974	1.8974	1.8974
3.2	0.7813	3.2	0.6429	3.2	1	1.2	1.7889	1.7889	1.7889
3	0.8163	3	0.6429	3	1	1.3	1.7321	1.7321	1.7321
3	0.7813	3	0.6429	3	1	1.4	1.7321	1.7321	1.7321
2.8	0.8163	2.8	0.6429	2.8	1	1.5	1.6733	1.6733	1.6733
5.2	0.7899	5.2	0.6429	5.2	1	1.6	2.2804	2.2804	2.2804
5	0.7899	5	0.6429	5	1	1.7	2.2361	2.2361	2.2361
4.8	0.7899	4.8	0.6429	4.8	1	1.8	2.1909	2.1909	2.1909
4.4	0.7899	4.4	0.6429	4.4	1	1.9	2.0976	2.0976	2.0976
4.2	0.7899	4.2	0.6429	4.2	1	2	2.0494	2.0494	2.0494
4.2	0.7899	4.2	0.6429	4.2	1	2.1	2.0494	2.0494	2.0494
4	0.7899	4	0.6429	4	1	2.2	2	2	2
3.8	0.7899	3.8	0.6429	3.8	1	2.3	1.9494	1.9494	1.9494
3.6	0.7899	3.6	0.6429	3.6	1	2.4	1.8974	1.8974	1.8974
4.6	0.7899	4.6	0.6429	4.6	1	2.5	2.1448	2.1448	2.1448
4	0.7899	4	0.6429	4	1	2.6	2	2	2
3.8	0.7899	3.8	0.6429	3.8	1	2.7	1.9494	1.9494	1.9494
3.6	0.7899	3.6	0.6429	3.6	1	2.8	1.8974	1.8974	1.8974
3.6	0.7899	3.6	0.6429	3.6	1	2.9	1.8974	1.8974	1.8974
3.4	0.7899	3.4	0.6429	3.4	1	3	1.8439	1.8439	1.8439
3.2	0.7899	3.2	0.6429	3.2	1	3.1	1.7889	1.7889	1.7889
3	0.8163	3	0.6429	3	1	3.2	1.7321	1.7321	1.7321
3.4	0.7899	3.4	0.6429	3.4	1	3.3	1.8439	1.8439	1.8439
3	0.7899	3	0.6429	3	1	3.4	1.7321	1.7321	1.7321
2.8	0.8163	2.8	0.6429	2.8	1	3.5	1.6733	1.6733	1.6733
3.8	0.7899	3.8	0.6429	3.8	1	3.6	1.9494	1.9494	1.9494
3.4	0.7899	3.4	0.6429	3.4	1	3.7	1.8439	1.8439	1.8439
3.2	0.7899	3.2	0.6429	3.2	1	3.8	1.7889	1.7889	1.7889
3	0.7899	3	0.6429	3	1	3.9	1.7321	1.7321	1.7321
3.2	0.7899	3.2	0.6429	3.2	1	4	1.7889	1.7889	1.7889
2.8	0.7899	2.8	0.6429	2.8	1	4.1	1.6733	1.6733	1.6733
2.6	0.8163	2.6	0.6429	2.6	1	4.2	1.6125	1.6125	1.6125
2.6	0.7899	2.6	0.6429	2.6	1	0.1	1.6125	1.6125	1.6125
2.4	0.8163	2.4	0.6429	2.4	1	0.2	1.5492	1.5492	1.5492
2.2	0.8163	2.2	0.6429	2.2	1	0.3	1.4832	1.4832	1.4832
3.2	0.7899	3.2	0.6429	3.2	1	0.4	1.7889	1.7889	1.7889
3	0.7899	3	0.6429	3	1	0.5	1.7321	1.7321	1.7321
3	0.7899	3	0.6429	3	1	0.6	1.7321	1.7321	1.7321
2.6	0.7899	2.6	0.6429	2.6	1	0.7	1.6125	1.6125	1.6125
2.4	0.8163	2.4	0.6429	2.4	1	0.8	1.5492	1.5492	1.5492
2.4	0.7899	2.4	0.6429	2.4	1	0.9	1.5492	1.5492	1.5492
2.2	0.8163	2.2	0.6429	2.2	1	1	1.4832	1.4832	1.4832
2	0.8163	2	0.6429	2	1	1.1	1.4142	1.4142	1.4142
1.8	0.8929	1.8	0.6429	1.8	1	1.2	1.3416	1.3416	1.3416
4.6	0.8098	4.6	0.6429	4.6	1	1.3	2.1448	2.1448	2.1448
4.2	0.8098	4.2	0.6429	4.2	1	1.4	2.0494	2.0494	2.0494
4	0.8098	4	0.6429	4	1	1.5	2	2	2
4.4	0.8098	4.4	0.6429	4.4	1	1.6	2.0976	2.0976	2.0976
3.8	0.8098	3.8	0.6429	3.8	1	1.7	1.9494	1.9494	1.9494
3.6	0.8098	3.6	0.6429	3.6	1	1.8	1.8974	1.8974	1.8974
3.4	0.8098	3.4	0.6429	3.4	1	1.9	1.8439	1.8439	1.8439
3.4	0.8098	3.4	0.6429	3.4	1	2	1.8439	1.8439	1.8439
3.2	0.8098	3.2	0.6429	3.2	1	2.1	1.7889	1.7889	1.7889
3	0.8098	3	0.6429	3	1	2.2	1.7321	1.7321	1.7321
2.8	0.8163	2.8	0.6429	2.8	1	2.3	1.6733	1.6733	1.6733
3.6	0.8098	3.6	0.6429	3.6	1	2.4	1.8974	1.8974	1.8974
3.2	0.8098	3.2	0.6429	3.2	1	2.5	1.7889	1.7889	1.7889
3	0.8098	3	0.6429	3	1	2.6	1.7321	1.7321	1.7321
2.8	0.8098	2.8	0.6429	2.8	1	2.7	1.6733	1.6733	1.6733
3	0.8098	3	0.6429	3	1	2.8	1.7321	1.7321	1.7321
2.6	0.8098	2.6	0.6429	2.6	1	2.9	1.6125	1.6125	1.6125
2.4	0.8163	2.4	0.6429	2.4	1	3	1.5492	1.5492	1.5492
2.4	0.8098	2.4	0.6429	2.4	1	3.1	1.5492	1.5492	1.5492
2.2	0.8163	2.2	0.6429	2.2	1	3.2	1.4832	1.4832	1.4832
3	0.8098	3	0.6429	3	1	3.3	1.7321	1.7321	1.7321
2.8	0.8098	2.8	0.6429	2.8	1	3.4	1.6733	1.6733	1.6733
2.8	0.8098	2.8	0.6429	2.8	1	3.5	1.6733	1.6733	1.6733
2.4	0.8098	2.4	0.6429	2.4	1	3.6	1.5492	1.5492	1.5492
2.2	0.8163	2.2	0.6429	2.2	1	3.7	1.4832	1.4832	1.4832
2.2	0.8098	2.2	0.6429	2.2	1	3.8	1.4832	1.4832	1.4832
2	0.8163	2	0.6429	2	1	3.9	1.4142	1.4142	1.4142
1.8	0.8163	1.8	0.6429	1.8	1	4	1.3416	1.3416	1.3416
1.6	0.8929	1.6	0.6429	1.6	1	4.1	1.2649	1.2649	1.2649
2.6	0.8098	2.6	0.6429	2.6	1	4.2	1.6125	1.6125	1.6125
2.2	0.8098	2.2	0.6429	2.2	1	0.1	1.4832	1.4832	1.4832
2	0.8098	2	0.6429	2	1	0.2	1.4142	1.4142	1.4142
1.8	0.8163	1.8	0.6429	1.8	1	0.3	1.3416	1.3416	1.3416
1.6	0.8163	1.6	0.6429	1.6	1	0.4	1.2649	1.2649	1.2649
1.4	0.8929	1.4	0.6429	1.4	1	0.5	1.1832	1.1832	1.1832
2.4	0.8098	2.4	0.6429	2.4	1	0.6	1.5492	1.5492	1.5492
1.8	0.8098	1.8	0.6429	1.8	1	0.7	1.3416	1.3416	1.3416
1.6	0.8163	1.6	0.6429	1.6	1	0.8	1.2649	1.2649	1.2649
1.4	0.8163	1.4	0.6429	1.4	1	0.9	1.1832	1.1832	1.1832
1.2	0.8929	1.2	0.6429	1.2	1	1	1.0954	1.0954	1.0954
4.2	0.8307	4.2	0.6429	4.2	1	1.1	2.0494	2.0494	2.0494
3.6	0.8307	3.6	0.6429	3.6	1	1.2	1.8974	1.8974	1.8974
3.4	0.8307	3.4	0.6429	3.4	1	1.3	1.8439	1.8439	1.8439
3.2	0.8307	3.2	0.6429	3.2	1	1.4	1.7889	1.7889	1.7889
3.4	0.8307	3.4	0.6429	3.4	1	1.5	1.8439	1.8439	1.8439
3	0.8307	3	0.6429	3	1	1.6	1.7321	1.7321	1.7321
2.8	0.8307	2.8	0.6429	2.8	1	1.7	1.6733	1.6733	1.6733
2.6	0.8307	2.6	0.6429	2.6	1	1.8	1.6125	1.6125	1.6125
2.8	0.8307	2.8	0.6429	2.8	1	1.9	1.6733	1.6733	1.6733
2.4	0.8307	2.4	0.6429	2.4	1	2	1.5492	1.5492	1.5492
2.2	0.8307	2.2	0.6429	2.2	1	2.1	1.4832	1.4832	1.4832
2.8	0.8307	2.8	0.6429	2.8	1	2.2	1.6733	1.6733	1.6733
2.6	0.8307	2.6	0.6429	2.6	1	2.3	1.6125	1.6125	1.6125
2.6	0.8307	2.6	0.6429	2.6	1	2.4	1.6125	1.6125	1.6125
2.2	0.8307	2.2	0.6429	2.2	1	2.5	1.4832	1.4832	1.4832
2	0.8307	2	0.6429	2	1	2.6	1.4142	1.4142	1.4142
2	0.8307	2	0.6429	2	1	2.7	1.4142	1.4142	1.4142
1.8	0.8307	1.8	0.6429	1.8	1	2.8	1.3416	1.3416	1.3416
1.6	0.8307	1.6	0.6429	1.6	1	2.9	1.2649	1.2649	1.2649
2.4	0.8307	2.4	0.6429	2.4	1	3	1.5492	1.5492	1.5492
2	0.8307	2	0.6429	2	1	3.1	1.4142	1.4142	1.4142
1.8	0.8307	1.8	0.6429	1.8	1	3.2	1.3416	1.3416	1.3416
1.6	0.8307	1.6	0.6429	1.6	1	3.3	1.2649	1.2649	1.2649
1.4	0.8307	1.4	0.6429	1.4	1	3.4	1.1832	1.1832	1.1832
1.2	0.8929	1.2	0.6429	1.2	1	3.5	1.0954	1.0954	1.0954
2.2	0.8307	2.2	0.6429	2.2	1	3.6	1.4832	1.4832	1.4832
1.6	0.8307	1.6	0.6429	1.6	1	3.7	1.2649	1.2649	1.2649
1.4	0.8307	1.4	0.6429	1.4	1	3.8	1.1832	1.1832	1.1832
1.2	0.8307	1.2	0.6429	1.2	1	3.9	1.0954	1.0954	1.0954
1	0.8929	1	0.6429	1	1	4	1	1	1
1.4	0.8307	1.4	0.6429	1.4	1	4.1	1.1832	1.1832	1.1832
1	0.8307	1	0.6429	1	1	4.2	1	1	1
0.8	0.8929	0.8	0.6429	0.8	1	0.1	0.8944	0.8944	0.8944
0.8	0.8307	0.8	0.6429	0.8	1	0.2	0.8944	0.8944	0.8944
0.6	0.8929	0.6	0.6429	0.6	1	0.3	0.7746	0.7746	0.7746
4	0.8528	4	0.6429	4	1	0.4	2	2	2
3.2	0.8528	3.2	0.6429	3.2	1	0.5	1.7889	1.7889	1.7889
2.8	0.8528	2.8	0.6429	2.8	1	0.6	1.6733	1.6733	1.6733
2.6	0.8528	2.6	0.6429	2.6	1	0.7	1.6125	1.6125	1.6125
2.4	0.8528	2.4	0.6429	2.4	1	0.8	1.5492	1.5492	1.5492
2.6	0.8528	2.6	0.6429	2.6	1	0.9	1.6125	1.6125	1.6125
2.4	0.8528	2.4	0.6429	2.4	1	1	1.5492	1.5492	1.5492
2.4	0.8528	2.4	0.6429	2.4	1	1.1	1.5492	1.5492	1.5492
2	0.8528	2	0.6429	2	1	1.2	1.4142	1.4142	1.4142
1.8	0.8528	1.8	0.6429	1.8	1	1.3	1.3416	1.3416	1.3416
1.8	0.8528	1.8	0.6429	1.8	1	1.4	1.3416	1.3416	1.3416
1.6	0.8528	1.6	0.6429	1.6	1	1.5	1.2649	1.2649	1.2649
2.2	0.8528	2.2	0.6429	2.2	1	1.6	1.4832	1.4832	1.4832
1.8	0.8528	1.8	0.6429	1.8	1	1.7	1.3416	1.3416	1.3416
1.6	0.8528	1.6	0.6429	1.6	1	1.8	1.2649	1.2649	1.2649
1.4	0.8528	1.4	0.6429	1.4	1	1.9	1.1832	1.1832	1.1832
1.2	0.8528	1.2	0.6429	1.2	1	2	1.0954	1.0954	1.0954
1	0.8929	1	0.6429	1	1	2.1	1	1	1
2	0.8528	2	0.6429	2	1	2.2	1.4142	1.4142	1.4142
1.4	0.8528	1.4	0.6429	1.4	1	2.3	1.1832	1.1832	1.1832
1.2	0.8528	1.2	0.6429	1.2	1	2.4	1.0954	1.0954	1.0954
1	0.8528	1	0.6429	1	1	2.5	1	1	1
0.8	0.8929	0.8	0.6429	0.8	1	2.6	0.8944	0.8944	0.8944
1.2	0.8528	1.2	0.6429	1.2	1	2.7	1.0954	1.0954	1.0954
0.8	0.8528	0.8	0.6429	0.8	1	2.8	0.8944	0.8944	0.8944
0.6	0.8929	0.6	0.6429	0.6	1	2.9	0.7746	0.7746	0.7746
0.6	0.8528	0.6	0.6429	0.6	1	3	0.7746	0.7746	0.7746
0.4	0.8929	0.4	0.6429	0.4	1	3.1	0.6325	0.6325	0.6325
0.2	0.8929	0.2	0.6429	0.2	1	3.2	0.4472	0.4472	0.4472
0	1	0	0.6429	0	1	3.3	0	0	0
									
									
									
									
									
									
									
									
									


==> Figures/Location_dependent_CC_data.tex <==
Single_User_Placement_NoCC	Single_User_Placement_NoCC_CDF	Multi_User_Placement_NoCC	Multi_User_Placement_NoCC_CDF	Uniform_Placement_CC	Uniform_Placement_CC_CDF	Proposed	Proposed_CDF	Unicasting_Uniform	Unicasting_Uniform_CDF
6.7665798400237	0.00159467390403103	7.20488093467022	0.00142789514699565	3.81486120235901	0.0813781080596828	4.41043707933024	0.00326506728224235	7.25149199958321	0.0656823478217474
6.88314334245288	0.00515359695618285	7.32894470887199	0.00334406022100219	4.10164669789508	0.0938323759777173	4.42321835985363	0.00358448640467762	7.56059052641765	0.0764724680820962
6.91955767725501	0.00723183101342571	7.35769590112305	0.00403393592634134	4.33519238490991	0.104971880448004	4.42484254358755	0.0036270239279784	7.85144031333482	0.0878097824406871
6.98824881964393	0.013225496499921	7.43734669354595	0.0066558637381852	4.3532828311251	0.105873097095654	4.43762501768104	0.0039779248271855	7.88890278012983	0.0893567760392136
6.99387320075346	0.013867308740545	7.44653836728838	0.00703930932634243	4.35852285497815	0.106135182245888	4.50179536509907	0.00624046652964291	7.89299588873376	0.08952701987471
7.00198329380272	0.0148399709707229	7.44996968047815	0.00718737335492005	4.38548277404311	0.107491020681613	4.52926108864348	0.00751596585014798	7.90691648071578	0.0901078214697288
7.01831005110055	0.0169770496384521	7.45421856479934	0.00737451808673584	4.39440581175126	0.107942505953927	4.53628724243031	0.0078770737889407	7.93948749140418	0.0914776942151952
7.02299384064228	0.0176367116588817	7.46890215940559	0.00805474475834525	4.46849788401661	0.111744211963451	4.58838983321569	0.0110644025225073	8.07368679036795	0.0972848350109748
7.02914210492301	0.0185357331675418	7.53333022926366	0.0117329439231327	4.49178776846777	0.112958782257362	4.6000270366275	0.0119132534254663	8.0748493424681	0.0973362967697556
7.05585186047477	0.0229074751183902	7.54528164001478	0.0125561677572623	4.50093542617883	0.113438401772831	4.60028543982424	0.0119327261638204	8.10465600230343	0.0986625522023635
7.0611349487962	0.0238679782202199	7.55577788505295	0.0133199393223468	4.51475010088303	0.114165466812219	4.68367403611898	0.0198445754343972	8.13072442799492	0.0998332753320492
7.06201448218226	0.0240311256200647	7.6252383802979	0.0194565307984852	4.52066005156361	0.11447751848324	4.70123978433135	0.0219863325391728	8.13177289367753	0.0998805728906604
7.06401992743469	0.0244066284765907	7.71234490337222	0.0304011720446763	4.56019584456445	0.116580672193455	4.73678437785601	0.0269205730543185	8.19788787870854	0.102896243428276
7.0736391978067	0.0262769016856825	7.71541786457847	0.0308656334065644	4.5638912319045	0.11677864400507	4.73781673120477	0.0270766886398375	8.20442695420272	0.103198064055041
7.07869822886484	0.0273076730416865	7.71937921413385	0.0314730206171481	4.58378525919844	0.117848515654769	4.745147859238	0.0282071913420956	8.26757364764165	0.106145820349488
7.10279810616522	0.0326915956856732	7.73723756579835	0.0343351142733644	4.64184249406901	0.121010341909892	4.75819354713791	0.030316029931436	8.27241231527437	0.106374178409193
7.10420078781472	0.0330301818503942	7.74188147416104	0.0351134441330331	4.66595913278883	0.122341136904764	4.77218291918537	0.032720911774425	8.29279848014767	0.107340187386123
7.11646334273904	0.036114904110002	7.76099650887814	0.0384710039389905	4.69321790966731	0.123857647877454	4.77740104115318	0.0336573119532485	8.34682496441907	0.109930808623551
7.12323845085796	0.0379179888360612	7.76291885039923	0.0388226812571776	4.71750410602176	0.125219824949284	4.78156551329851	0.0344203596733012	8.34891849024152	0.110032090419713
7.1287087068337	0.0394268258330436	7.77257830478362	0.0406296381495431	4.72932128199288	0.125886402550416	4.787031837874	0.0354434594423933	8.3728047450098	0.111192415420164
7.12911183190665	0.0395399236417357	7.77463826200743	0.0410236841861048	4.77362672831368	0.128407576777452	4.83085763268726	0.0445776598037255	8.42220412755868	0.113619830389377
7.12940558796271	0.0396225037714532	7.77500279571964	0.0410937369954422	4.82793082710836	0.131545249258275	4.8469988398097	0.0483860264745402	8.51829916013864	0.118449515367193
7.1461001235681	0.0445509517362565	7.78739669369857	0.0435337685852261	4.8368936941293	0.132068165953216	4.84847552646604	0.0487470520998934	8.52135392921444	0.118605390655429
7.15933228552802	0.048798455310701	7.80254022622811	0.0466724283539409	4.85750648129157	0.133276202502571	4.85362398306541	0.050022631534504	8.55506605064879	0.120335245517199
7.1600872592595	0.0490502406575772	7.81079048160266	0.0484573119377221	4.9004090976618	0.135814881804631	4.86573415404114	0.0531280305512372	8.57023293471611	0.121119265719785
7.16767180698552	0.0516376766623057	7.82020051048056	0.0505592947169287	4.90395745421815	0.136026321863296	4.87462025855854	0.0555024375268077	8.58301541751964	0.121782814042084
7.17089726621622	0.052770406262646	7.82392797606663	0.0514117488732999	4.90567709382756	0.136128873056903	4.88356949585245	0.0579776022822034	8.59727236378956	0.122525911098772
7.18639378577332	0.0584898427930171	7.83210567905315	0.0533219965972099	4.92221127866362	0.137117594218668	4.89377201009829	0.0609043277615021	8.6058881436566	0.122976519898573
7.19312583832831	0.0611214258916265	7.83713437950629	0.0545243185333302	4.94817981571348	0.138680358975014	4.89455057711716	0.0611323300952266	8.62727864319595	0.124100270768868
7.19628842815601	0.062389219508635	7.86103205682441	0.060533633152911	4.96510249985325	0.139705256866996	4.89550573639242	0.0614129578077783	8.63249406656926	0.124375349298552
7.20399981974143	0.0655664434606128	7.86172021106747	0.0607140593968259	4.96518825647227	0.139710463672965	4.89681462404806	0.0617991446854384	8.63607767277072	0.124564607414648
7.20496955973839	0.0659747187772367	7.86229460217357	0.0608649800542992	4.97578072107511	0.140354611371476	4.89755312515499	0.0620178742357517	8.66166544880762	0.125921805344465
7.21096278827407	0.0685418080179044	7.86810564926636	0.0624083694567995	4.98532047181848	0.140936465058123	4.89780238451029	0.0620918361699763	8.75361997533723	0.130884118835104
7.21371177175375	0.069744759804349	7.86989095996687	0.0628886187763059	4.99265797745606	0.14138510992806	4.90124835256521	0.0631214137899665	8.77498383980067	0.132056104938859
7.21903727330642	0.0721213474125345	7.87863668893491	0.0652829368167405	5.00758235179196	0.142300630637753	4.91453299225238	0.0672153928864765	8.79662022974613	0.133250396884392
7.22247335810865	0.0736873900539216	7.88593392172328	0.0673343166569179	5.04771179571598	0.14478218780019	4.91588859328834	0.0676444400492912	8.81785204376825	0.134429561344595
7.22349669724903	0.0741587791502074	7.88636856590698	0.0674580575360904	5.049185965365	0.144873900297964	4.92427123465322	0.0703446885420966	8.83015514060463	0.135116115079744
7.22737812712077	0.0759676679477455	7.88761822121301	0.067814806819301	5.07035410652526	0.14619514716996	4.92452549551267	0.0704278686491661	8.86889787110926	0.137293776847359
7.22815619982935	0.0763342873382303	7.89723990263917	0.0706105722534028	5.08349261267876	0.147019268184765	4.93432794294177	0.0736926777494787	8.91453607634781	0.139889617075198
7.22844670783178	0.0764715161924263	7.8976376795725	0.0707280328868864	5.09914632432772	0.14800521657045	4.94944128216001	0.0789513213323163	8.91633300403616	0.13999250198389
7.23250991639719	0.0784105965288041	7.90049200365132	0.071575302757679	5.10411414104672	0.148319037287475	4.95181602798227	0.0798028274119349	8.93060238353239	0.140811334964367
7.23352144867605	0.0788990755547158	7.92629510246337	0.0795915760312302	5.10732699875505	0.148522232773706	4.95408873000047	0.0806242313220593	8.9362853775596	0.141138350475598
7.23472738391556	0.0794844420456874	7.93860809198093	0.0836484207506287	5.11291915783773	0.148876349675901	4.967714705218	0.08568336092197	8.93690577552344	0.141174081076676
7.25174783527187	0.0881003105864889	7.94354215191541	0.0853169857805814	5.12617828272557	0.149718221192933	4.97175079767482	0.0872266052453735	8.94668021831879	0.141737830426017
7.25323820549439	0.0888866826324466	7.95680791795425	0.0899266030093423	5.14192361946663	0.150722069073475	4.99071166500976	0.0947550333113318	8.96820258025161	0.142984519904114
7.25539526117377	0.0900340596075704	7.96537052751129	0.0929987141836178	5.14270328132183	0.150771892793422	4.99245076283636	0.0954688109149727	8.97905012828284	0.143615667595356
7.25551751423119	0.0900994162257629	7.96927542516298	0.0944252033603931	5.15896376848498	0.151813506444838	5.0065115837441	0.101385619824097	9.0049482651732	0.14513010404351
7.2595305481817	0.0922644026559102	7.98349859350342	0.0997574536087363	5.16089131815591	0.151937297587352	5.00741423382929	0.101774384105652	9.0247848685178	0.14629732560213
7.26128963390443	0.0932254555728491	7.99114574049264	0.102713722942312	5.16711042392022	0.152337158228256	5.00989121660735	0.102846773562536	9.03385441563488	0.14683308835479
7.26214970484043	0.0936980274645596	7.99565000033297	0.104484526257217	5.17986484215502	0.153159393589157	5.01143668878622	0.103520019202649	9.06734320586325	0.148822752996301
7.26385350727719	0.0946394114404869	7.99762706815894	0.105268736337498	5.20688416869972	0.154910938592374	5.01370986504471	0.104516073892133	9.07067327997222	0.149021582496809
7.26386742165423	0.0946471279991808	8.0003254719659	0.106345926621941	5.21944874694769	0.15572993441257	5.01491720421632	0.10504791740166	9.09828432377945	0.150676994951647
7.26526818296247	0.0954263297658697	8.00132593164057	0.106747321384706	5.24658238620804	0.157508307972795	5.0149452287553	0.105060285676662	9.11275710766287	0.151549579876586
7.26542219716899	0.0955122905736551	8.00315715359783	0.107484856393107	5.28902569881473	0.160316758235827	5.01735469713492	0.106127618249862	9.11685290227587	0.151797129876568
7.26704260580357	0.0964201545072698	8.00383377947736	0.107758298359571	5.30953231604419	0.161685323969203	5.01764271976994	0.106255727172398	9.12857218590951	0.152506927406201
7.2679147698022	0.0969114177779338	8.00531768098279	0.108359734985338	5.34727409659667	0.164223969961029	5.02026658751822	0.107427937360797	9.14215208795047	0.153332166654218
7.27351801093367	0.100111439047375	8.00897685362733	0.109853138862899	5.35854774401792	0.164987262317793	5.0246207421026	0.109393668201578	9.1464670683944	0.153595002613109
7.28215729697239	0.105195434740399	8.01298220662844	0.111504698192797	5.36136711458252	0.165178508821919	5.0260057522894	0.110024329286861	9.19036631504636	0.156285962061154
7.28291927466132	0.105652646308673	8.01536736480156	0.112496590727346	5.38055346133726	0.16648378609868	5.0355325567691	0.114433092807078	9.21737190112387	0.157956701603354
7.28534701473984	0.107118947729355	8.0253514631117	0.116716963373178	5.38479318996409	0.166773117356086	5.03978276875883	0.116440028685562	9.22443833458259	0.158395805345318
7.29014238895495	0.110058253773571	8.02778500806732	0.117762445734736	5.38577389421193	0.166840089603486	5.05692872673832	0.124789426087119	9.26894445425763	0.161179774102303
7.29338489056594	0.112078249484871	8.03074033518288	0.119040981455834	5.40630275348347	0.168245986157591	5.05737213007301	0.125010758061017	9.29714566220716	0.162960253577226
7.29481333281172	0.112976492157697	8.03162690857881	0.119426435539877	5.42152258798226	0.169293204876129	5.06330802745943	0.128000182494546	9.29963117172934	0.16311778672298
7.29533640352931	0.113306694815829	8.04031941483783	0.123252347666429	5.43730339639634	0.170383430604768	5.06639155745488	0.129572550991109	9.33366379496964	0.165284746793739
7.2994265231908	0.115912447583323	8.04453219870479	0.125137135763466	5.43860239345966	0.170473372403356	5.07025415181531	0.131560993948826	9.33663517261104	0.165474823651724
7.29982478363641	0.116168428125088	8.04704810722993	0.12627229890532	5.45198286881382	0.171401597773522	5.07272944011296	0.132846277528333	9.35235592624767	0.166482820741368
7.30171348875748	0.117387849379666	8.04872543865872	0.12703307653041	5.45526016552731	0.171629440796428	5.07874546593068	0.136006031387436	9.35290371988562	0.166518015976436
7.30185129853845	0.117477178228542	8.05406557636053	0.129476392816741	5.45910368642657	0.171896895062874	5.08081746657301	0.137106109417375	9.38073241039758	0.168312301873592
7.30411994190129	0.118954643769396	8.05937045657236	0.131935626808519	5.46003796005741	0.171961947375501	5.08154011866585	0.137491209741594	9.41257180916149	0.170380376949711
7.30738916185561	0.121106742265765	8.06858390074574	0.13628295906473	5.48873431069795	0.173967690846288	5.08268030322298	0.138100313006436	9.43130542232613	0.17160476040977
7.31321569363733	0.125009898479826	8.07239432585446	0.138109231111002	5.50112184458714	0.174838100732343	5.0835911117217	0.138588200404521	9.43442416286962	0.17180913821966
7.31372979852659	0.125358465386836	8.07511023487275	0.139421062253333	5.51757395166752	0.175998372986664	5.08430134677077	0.138969461767739	9.44681322857826	0.172622555004461
7.31420441665618	0.12568086176575	8.07570738131661	0.139710627339841	5.5281539303384	0.17674708754067	5.08744000634613	0.140662871877284	9.48071976426841	0.174861254540899
7.31586314502663	0.126812136577298	8.08225393422432	0.142911959589411	5.53087830672491	0.176940209332334	5.09129973334451	0.14276444848051	9.48561602931139	0.175186049276093
7.31757737857474	0.127988695888451	8.08582792984444	0.14468044095789	5.53560834718965	0.177275822441567	5.09143086096293	0.142836216808602	9.48747152910393	0.175309234142589
7.31759878424944	0.128003435395566	8.08995586288063	0.146741292734138	5.5447089484308	0.177922672218524	5.09465036748097	0.144605957005071	9.49357919553476	0.175715104128996
7.32660132091286	0.134307182536475	8.09635019684575	0.14997234395072	5.54836597159037	0.178183023720876	5.0982189670948	0.146584783055985	9.49834476288476	0.176032201334907
7.32865845956443	0.135777056650156	8.10604691549942	0.154961959263702	5.55045530956312	0.178331876004182	5.10105666200309	0.148171227394942	9.51017100424221	0.176820674338241
7.32883645111847	0.135904751704127	8.10864456527644	0.156317034095464	5.55874244080877	0.178923053780562	5.10204039164085	0.14872386393144	9.51339540126911	0.177036036360006
7.34375727028708	0.146902349929795	8.1113042887707	0.157712553015883	5.5606013519098	0.179055831795891	5.10555008881318	0.150706744412528	9.51868534230163	0.177389717784538
7.34601811150958	0.148619402969853	8.11469786623179	0.159504960858812	5.57919464934521	0.18038732026167	5.1072907594118	0.151696675398135	9.52390323125135	0.177739018567458
7.35481027738629	0.155423954696054	8.11770418366543	0.161103922327293	5.58578549719661	0.180860786297163	5.10788293088102	0.152034430220738	9.52736287975184	0.177970856651928
7.35951615264812	0.159149151913175	8.11907678495564	0.161837429734986	5.59042279187586	0.181194381520517	5.10902985812064	0.152690018686796	9.53129608947057	0.178234660554853
7.36284777934432	0.16182155796188	8.11910446165308	0.161852242292063	5.59823625394181	0.181757333269395	5.11314063763285	0.15505514238539	9.57648844488367	0.181283415589209
7.36757819024733	0.165665912226237	8.12086397715393	0.162795747322586	5.64644893087063	0.185255166718956	5.11533883843286	0.15632974417317	9.58372934225278	0.18177491720422
7.3676871852049	0.165755181727517	8.1237774872249	0.164365907848524	5.68526888421799	0.188101722219448	5.11938329962878	0.158692859083748	9.59176695668043	0.182321474080151
7.36780222114241	0.165849432663326	8.1253670820257	0.165226704524618	5.69765229710067	0.189015411738566	5.12251704718439	0.160539878514649	9.62017636001701	0.184261527364106
7.36853583037	0.166451306091168	8.12696417489353	0.166094494415936	5.70296279288575	0.189408073984094	5.12679347084929	0.163082953486305	9.62654040753967	0.184697877478094
7.37343257020244	0.17050478959671	8.13183730945744	0.168760504255763	5.75914493899787	0.193592915147295	5.12955984293562	0.164741912404839	9.6583226979939	0.186886628408739
7.37738532315131	0.173822559788894	8.13357727491465	0.169719035609652	5.76363656013772	0.193929899518763	5.13980761163826	0.17098225669169	9.66103284533912	0.187074007907828
7.38072599971761	0.176658373289531	8.14352147485654	0.17526403367358	5.768369234969	0.194285355469875	5.14026809949776	0.171266174669851	9.68162202455873	0.188501335297423
7.38215850752842	0.177883302982805	8.14453241296868	0.175834107355306	5.78318592620312	0.195400752161821	5.14608540547009	0.174878815559662	9.74132437061398	0.192677976267731
7.38250763268781	0.178182647973574	8.1523512998212	0.180282814110358	5.78460477735501	0.195507766605046	5.14669513748784	0.175260249339026	9.750060717593	0.193293859897102
7.38377502799182	0.179271997515594	8.15646005058728	0.182648628545576	5.79510867624233	0.196301111944063	5.14944427835749	0.176986591260994	9.76721687940149	0.194506803752943
7.38416165326231	0.179605140990877	8.16674748797695	0.18865666148529	5.7978347828369	0.196507329651642	5.15025337026241	0.177496705689143	9.77531034498059	0.195080617939746
7.38553041411327	0.180787685495648	8.17623316632671	0.194303087170048	5.80668355608505	0.197177603620455	5.15123673381629	0.17811794256468	9.78556318232192	0.195809003903639
7.39071008344315	0.185306713576154	8.18152087751662	0.197494834951893	5.83494149330624	0.199327320969871	5.15367335645809	0.179663168541801	9.79686101274023	0.196613537238578
7.39088478818156	0.185460348341118	8.18485837984759	0.199525626448639	5.83724824088782	0.199503427221728	5.16672022278073	0.188079670153384	9.80566179057992	0.197241637615723
7.39196412051088	0.186411261727108	8.1851981457686	0.199733068541295	5.84274700859402	0.199923602473642	5.18102189517825	0.197580263232024	9.81300383972746	0.197766557989957
7.39274373799235	0.187099995454684	8.18940241172421	0.202310679570519	5.84559227103128	0.200141225191119	5.18741626512434	0.201920259772104	9.81414358969743	0.197848120126888
7.39647335519692	0.190416560878844	8.19081920637021	0.203183770448806	5.91496960577586	0.205491567174111	5.19381526443957	0.206320031044888	9.81878253397562	0.198180299239599
7.40078265533543	0.194293254429589	8.19196111032447	0.203889095832745	5.93381559493259	0.206959497479068	5.1987227502406	0.209732456059308	9.84344548899282	0.199951976386594
7.40125429796096	0.194720447814201	8.19385798848481	0.205063969838798	5.93970029533995	0.207419130121148	5.20371262187289	0.213235962583162	9.86332262132717	0.201386768558404
7.40310249727143	0.196399965928749	8.19869346976767	0.208077078509626	5.93970584329288	0.207419563736188	5.2065399702612	0.21523616572598	9.86417522207306	0.201448449592006
7.40457425000946	0.197743654229137	8.19883256306292	0.208164135894595	5.94474356381965	0.207813521320182	5.20840625411399	0.216562410324304	9.88093618886262	0.202663312025895
7.40677693127959	0.199765017294974	8.20695623512424	0.213285866130348	5.95636103858389	0.208723708843815	5.20948290337302	0.217329659373656	9.90878309040042	0.204691354544417
7.41000049623492	0.202745534455732	8.21275216013628	0.216984515166447	5.97935373443171	0.210532015087542	5.21175223721103	0.218951978353114	9.95211251374801	0.207870860359685
7.41097654239108	0.2036532037229	8.21354205488147	0.217491438281034	5.99280445020941	0.211594122356121	5.21253638820563	0.21951417356048	9.95239901796828	0.20789198058636
7.41815316468756	0.210401141479758	8.21516570248569	0.218535574946688	5.99655507350069	0.211890840704625	5.21353653399344	0.220232427563784	9.962947042724	0.208670430870491
7.41914631366692	0.211345196624529	8.21718243402853	0.219836506610066	6.00087953860996	0.21223325862128	5.21615463186714	0.222118980515802	9.96359536792632	0.208718333623917
7.41933385743449	0.21152374773948	8.21863506939025	0.220776304731629	6.00587150813506	0.212628932494437	5.21728592593125	0.222937015562231	9.97904832686314	0.209862022203486
7.42083031867567	0.212951615100131	8.22055177354651	0.222019850769249	6.01005100164127	0.212960538907528	5.22170765933062	0.226150768574643	10.0022603578482	0.211586872110116
7.42281676672685	0.214855671548371	8.22450475937619	0.224597111691023	6.01259758125643	0.213162735691013	5.22488951982824	0.228479477948009	10.0475688714672	0.214977485713556
7.4265874071439	0.21849699357974	8.22947088747135	0.227858843513254	6.03949467550459	0.215305174735977	5.22783573166448	0.230647682478984	10.0537389108959	0.215441642591941
7.42766583883616	0.219544937799921	8.23029466947081	0.228402465752886	6.06253466080157	0.217150278725931	5.23014038676016	0.232351729209941	10.0712764675462	0.216764120002766
7.4283107782834	0.22017302169163	8.23338010540608	0.230445040209949	6.07644878429907	0.218268969184543	5.23386255516896	0.235118606412244	10.0903214550598	0.218205572999023
7.42957056992572	0.221402856319036	8.23415894603092	0.230962246140282	6.13631473221779	0.223119882832796	5.23662145092621	0.237181121155607	10.1281945792642	0.221088420641905
7.43121651977003	0.223015569529678	8.23512692891664	0.231605958325252	6.14376020081896	0.223727448612463	5.23777594239227	0.238047144907427	10.1499798747205	0.222756511630296
7.43161753602084	0.22340949922128	8.23540012933692	0.231787818382454	6.14967054763209	0.224210414188962	5.24023573557503	0.239898086957578	10.1881689447488	0.225697869856885
7.4324864398784	0.224264405083004	8.24073219333948	0.235353073450776	6.15198990759068	0.224400102936122	5.24037559714937	0.240003565155437	10.1995401189611	0.226577915215711
7.4325783973851	0.224354989718368	8.24099247791608	0.235527882781006	6.15718369927233	0.224825207140496	5.24273709966116	0.241788331632374	10.2000922209636	0.226620693106651
7.43370058756876	0.225462098120682	8.24286595620934	0.236788237870509	6.16001427580393	0.225057077757256	5.24423194169142	0.242921809034646	10.2058781980614	0.227069275511263
7.4339668381474	0.225725223587439	8.24425374755287	0.237724240277354	6.16898544842327	0.225792858476295	5.24547371140243	0.243865573689958	10.2065507221514	0.22712144824936
7.44305867646505	0.234813943709026	8.2473449436541	0.239816388318605	6.17649868076068	0.226410110060542	5.25283681763186	0.249502076885751	10.2368323961547	0.229477616098624
7.44378333973631	0.2355469611272	8.24792236981076	0.240208305720082	6.19733146556627	0.228126607962973	5.25467889605334	0.250922947729003	10.259724118873	0.231267837424402
7.44402182170812	0.235788468202727	8.25086206239291	0.242208969366764	6.20235626749592	0.228541714488685	5.25656389119109	0.252381343464924	10.277026660094	0.232626116650376
7.44417440864452	0.235943062272705	8.26043082899011	0.24878326602046	6.22896275768312	0.230746774306376	5.25768058059352	0.253247413978442	10.2869065343343	0.23340368845598
7.4456634521091	0.237454621438676	8.26150158673122	0.249524804254998	6.23141239685504	0.230950388199583	5.26367119917	0.257920102399225	10.3071721846673	0.235003150846419
7.44843773958079	0.24028498292678	8.2665976422752	0.253070040555011	6.25344857736451	0.232786537477405	5.26473672347931	0.25875587330532	10.3157021644864	0.235678184343664
7.44922228861447	0.241088710668215	8.27140383903648	0.256437750103047	6.25661659044121	0.233051175244747	5.2659759408893	0.259729644853923	10.3158593095738	0.23569063029363
7.44992408702409	0.24180890164309	8.27457526520817	0.258672693633232	6.25912133913981	0.233260525883923	5.26991721073752	0.262839202131849	10.331385421551	0.236922089685545
7.45370315861772	0.245707006441666	8.27901051082977	0.261815093582672	6.26598149566613	0.233834442061237	5.27736053497057	0.268763274564882	10.3328723443136	0.237040210831215
7.4548170648572	0.246862403871176	8.27932395807357	0.262037911481806	6.27321799482858	0.234440689960822	5.2785656830136	0.269728711369476	10.3511146253822	0.238492008660341
7.45690585377598	0.249036812720982	8.28114786200507	0.263336382074671	6.29302952180269	0.236104869575123	5.27944627318913	0.270435243387248	10.3657916671006	0.239663594496563
7.45816485626535	0.250352327495872	8.28217542858063	0.264069369752997	6.30260343692874	0.236911410375303	5.28390532381763	0.274027052647801	10.3798191353969	0.240786257763377
7.46024933890936	0.252538447958505	8.28289216274936	0.264581247986345	6.30589168115344	0.237188772855186	5.29328331178368	0.281657200434387	10.390998677502	0.241683037457771
7.46087343687131	0.253194927470238	8.28478386922259	0.265934689643071	6.35478407653838	0.241333806198537	5.29414718831965	0.28236519073101	10.432640521515	0.245039281746849
7.46302905665381	0.255469277232727	8.28492494305433	0.26603576279945	6.35821912430473	0.241626497494851	5.29417492472362	0.282387936287382	10.432660975342	0.245040936419808
7.46313208935067	0.255578251568872	8.28867846586916	0.268732121956308	6.3638335511469	0.242105302527041	5.29569844626066	0.283638669426257	10.4532870878706	0.246712601956541
7.46346336427405	0.25592879476019	8.28945157843771	0.269289190920753	6.40633235405609	0.245746280690189	5.29600320940542	0.283889182505078	10.4550451135654	0.246855364932386
7.46964678991867	0.262517627827804	8.29366914994208	0.272338337613197	6.42109372537719	0.247017768758867	5.29778846839019	0.285358775499942	10.4767375617126	0.248620564276346
7.47118457080306	0.264169609930533	8.29716781623181	0.274880691847889	6.42148620507628	0.247051623429339	5.2996834451804	0.286922639339419	10.5064592002163	0.251050005111822
7.47770714260504	0.271234940780711	8.30028468082811	0.277155412953777	6.44063309523699	0.248706213639449	5.30015897974006	0.287315719226141	10.5076868108813	0.251150619169458
7.47787875902917	0.271422101934993	8.30179751203615	0.278262803693307	6.44438200717775	0.249030867617709	5.30218700400736	0.288994950960123	10.5197362925027	0.252139316720558
7.4783213498235	0.271905078615159	8.30234151575448	0.278661540463284	6.44662682908014	0.249225375998971	5.30297181980212	0.289646025972867	10.5307150909006	0.253041945634064
7.47885769643375	0.272490938621508	8.30369069140442	0.27965164060376	6.45331757552084	0.249805591886942	5.30331711417308	0.289932696526403	10.5620360611275	0.255626332798674
7.48049104601053	0.274278924484584	8.30393760040873	0.279833020821679	6.45778418382613	0.250193331207982	5.30365489505687	0.290213257898396	10.5701210186484	0.256295678330662
7.48235082834629	0.276321808621609	8.30685558947776	0.281980896992821	6.49861811405891	0.253752807468654	5.30401159333044	0.290509670086745	10.5786772597839	0.257005034695088
7.48350018312363	0.277588042380763	8.30788971042491	0.282743994956574	6.5055610646883	0.254360655462537	5.30441784164715	0.290847430267002	10.5863021978638	0.257638040772494
7.48796952076208	0.282538645875237	8.31542206847186	0.288331993508058	6.50656185940611	0.254448336874759	5.30491850711303	0.291263942444436	10.5964484713595	0.258481616358688
7.49475630232616	0.290136426334736	8.31624447565516	0.288945248692874	6.51084867402292	0.254824091503118	5.30517790413801	0.291479848711201	10.5964619431803	0.258482737375308
7.49600332774295	0.291542811777734	8.32108388244814	0.292566284985047	6.51107633418013	0.254844054849192	5.30531814696782	0.291596609372923	10.6018446675128	0.258930845851346
7.49705856930512	0.292735382443355	8.32661960573713	0.296733999091664	6.51910508654355	0.255548613204034	5.30858507114483	0.294322671359857	10.6252633277243	0.260885101925829
7.49836423762084	0.294214098092006	8.33437267977088	0.30261635147319	6.52364825252619	0.255947746335775	5.31249703875751	0.297602381629041	10.6514865224278	0.263082361369491
7.50165465318111	0.297955831232669	8.33828708046361	0.305605970673841	6.52679472637634	0.256224365671158	5.31304980258697	0.298067148898617	10.6533303465082	0.263237211736922
7.50218169136041	0.298557168541856	8.33957230677815	0.306590407186794	6.55248449299893	0.258488675658668	5.31524988286989	0.299920259223373	10.6735220057651	0.264936014211136
7.50313169674813	0.299642492702276	8.33980465870362	0.306768529617016	6.55978091560828	0.259133671041262	5.32646941879922	0.309450384265584	10.6835580835572	0.265782456283082
7.50314382981482	0.299656365556902	8.34100888622501	0.307692428390715	6.58318094414392	0.261207805681443	5.32719065160922	0.310067516567322	10.6849114025082	0.265896699901143
7.50767155338314	0.304853504356542	8.34463454580693	0.310481434546447	6.64896956337508	0.267084551824786	5.32784098366501	0.310624440868855	10.6898640274498	0.266314999491683
7.50915014160628	0.306559334273421	8.34965990360392	0.314365204932181	6.64966803664852	0.267147301110003	5.33489311386746	0.316691336794912	10.6933481066454	0.266609464859703
7.51061857671208	0.308257608778814	8.35270003603585	0.316724776089938	6.64973460239447	0.267153281616944	5.34273024219747	0.323491822159464	10.7076248678691	0.267817816767846
7.51785266425628	0.316683458478942	8.36072540626377	0.32298931846435	6.65379397141565	0.267518117667025	5.34783460284435	0.327953117113148	10.733266958332	0.269995009176082
7.52046878158861	0.31975444268855	8.36083266540194	0.32307339032403	6.66361520404689	0.268401839522349	5.35022255902913	0.330048739216546	10.7338495889767	0.270044581301902
7.52224097486712	0.321841828480165	8.37025656897819	0.330494907101313	6.67537300039678	0.269461742113628	5.35585307181713	0.335011025845109	10.7492564789005	0.271357100147926
7.52458709370253	0.32461387753329	8.37094565604317	0.331040247234875	6.67967623340707	0.269850179356881	5.3579408009977	0.336858387366099	10.7504370085622	0.271457800889735
7.52573661881965	0.325975662200179	8.37148314722026	0.331465864174786	6.68261967726101	0.270116034721046	5.35807501270213	0.336977282144853	10.7779378903457	0.273808917262371
7.52590729563845	0.326178053075406	8.37251483420086	0.33228342394745	6.69795838748262	0.271503562249577	5.36019717749232	0.338859412993573	10.8101289827012	0.276573742102519
7.52990337501445	0.330931183632624	8.37534643301196	0.334531418108368	6.69940475617838	0.271634582541736	5.36306341728535	0.34140784999696	10.8121910577027	0.276751314686184
7.53046592909017	0.331602529010823	8.37580347264502	0.334894819261614	6.70077434410811	0.271758676606594	5.36307807369005	0.341420900053292	10.8216520936547	0.277566753302876
7.53076198007174	0.331956050286535	8.37586700285344	0.334945345623552	6.73586886508825	0.274948072355369	5.36314281175454	0.341478545065817	10.8289458512362	0.278196196422564
7.53084076996329	0.332050160332028	8.38300360554979	0.340640003366262	6.75461863781433	0.276659581246124	5.36586624156926	0.343906916664665	10.8316282051079	0.278427855497273
7.53304814669196	0.334691033971553	8.38859061017031	0.345123729637881	6.7684688333941	0.277927192799875	5.36702632660354	0.344943283242682	10.8343703569025	0.278664776089902
7.53549594603746	0.337629132223332	8.39171034591154	0.34763694644883	6.77044910897879	0.278108664936404	5.36727704934553	0.345167420680496	10.8375448809076	0.278939175972107
7.53583696468736	0.33803924923383	8.39273663338342	0.348465182217941	6.77321424159186	0.278362157904103	5.36919273804471	0.34688176817041	10.8502812809498	0.280041406147287
7.53745162231776	0.339983678022344	8.40015434793015	0.354472716212594	6.79732885526487	0.28057762102636	5.36936681056111	0.347037701564202	10.87885663752	0.282522021814061
7.54105586181131	0.344339354019776	8.41149425947498	0.363726739138039	6.81255991446327	0.281981314784728	5.37050733346773	0.348060016796786	10.8811090222637	0.28271799878318
7.54267002176252	0.346296801264856	8.41355334941827	0.365415824461719	6.8141000033423	0.282123437395998	5.37595507637878	0.352958272176915	10.8819148194157	0.282788125971227
7.54340959233053	0.347195035274391	8.41616381887298	0.367560964276822	6.81761123408073	0.282447589966549	5.38030095270304	0.356883398125449	10.8873203605978	0.283258777165601
7.54739874060336	0.3520546954382	8.42141877599244	0.371891690612718	6.82466740684102	0.283099548426866	5.38031400631749	0.356895211042086	10.8902318314806	0.283512429519225
7.5511661464401	0.356666533693475	8.42437967429735	0.374339031417769	6.84168627454169	0.284674979619232	5.38726154152921	0.363201621207509	10.9024408820221	0.284577286667719
7.56308616259189	0.371394031642942	8.42498351003726	0.374838759829217	6.84213273700341	0.284716364782496	5.3885755537488	0.364398618248903	10.930674040551	0.2870470339712
7.56354725043012	0.371967681004077	8.43343088436721	0.381851410134092	6.84672423747321	0.285142143807647	5.39015943314878	0.365843208970429	10.9319050934141	0.287154953129551
7.56410205762688	0.372658305453019	8.43626378066101	0.384211997680015	6.8814369246764	0.288370901156967	5.39095784824423	0.366572133520015	10.980498371073	0.291430103466568
7.56682321304214	0.376051494522353	8.43779459080034	0.385489382658422	6.88552861217131	0.288752617112305	5.39176856419605	0.367312781068543	10.9812175494706	0.291493597883982
7.56837898974408	0.377995829051444	8.44245686782572	0.389387426014257	6.89452346569056	0.289592587637103	5.39337681560294	0.368783494353446	10.98979896932	0.292251726780097
7.56861935020149	0.378296497137132	8.44457557390365	0.391162548028055	6.90090174394378	0.290188907591452	5.39549493641201	0.370723405533266	11.0002393086119	0.293175317454995
7.57118104836818	0.381505483133694	8.44854503629116	0.394494378012433	6.90366145895824	0.290447097907734	5.39608087970218	0.371260633309739	11.0082091044717	0.293881264393387
7.57172908370297	0.38219306301107	8.45058557826143	0.396210164041732	6.94391078016654	0.294224860934249	5.39716075001158	0.372251379584523	11.008663611142	0.293921547278464
7.5740009704388	0.385047374861283	8.4537224478896	0.39885170954688	6.95926162490998	0.295671632370181	5.40012806926926	0.374978139137703	11.0969505468181	0.30179434929299
7.58024776562866	0.392927348004214	8.454967369848	0.399901346307468	6.97896847272455	0.297533721886963	5.40189514630541	0.376604943521219	11.0978340834759	0.301873613896573
7.58067580723937	0.39346894844082	8.45731061042201	0.401878970870508	6.99171228457442	0.29874072113046	5.40511810622644	0.379577692996669	11.0990450016336	0.301982264025834
7.58155391082299	0.394580655971347	8.46042804560576	0.404513883704083	6.99946319605578	0.299475916688468	5.40589414745487	0.380294559373791	11.106155251007	0.302620588125218
7.58293308845762	0.396328470658559	8.4611986935435	0.405165922486058	7.00542028642266	0.300041520138627	5.40753819277835	0.381814598735356	11.1724403731256	0.308600196075115
7.58314251673423	0.39659405977826	8.46271173894994	0.406446862019402	7.0072041994805	0.300210989991795	5.40963556887811	0.383756420738019	11.1777408799427	0.309080584838569
7.58406851924527	0.397768955117703	8.4700086202815	0.412638209708319	7.01895250608391	0.301328145990262	5.41271635596288	0.386614005813402	11.1792316653096	0.309215754687446
7.58691341968092	0.40138427430898	8.47007263411401	0.412692623659926	7.03956487736213	0.303292701831772	5.41379997979127	0.387620593727875	11.1857709852539	0.309808981250668
7.58832887258953	0.403186212765124	8.47116499346843	0.413621424317365	7.04106125176992	0.303435543255592	5.41434902391523	0.388130894678022	11.1886205490827	0.310067639872256
7.59260013733675	0.408636060216809	8.47679102140435	0.418412616450727	7.0597798585301	0.305224923635643	5.41449694820328	0.388268413799121	11.2184191482361	0.312778110150918
7.59331095699673	0.409544766309283	8.47729736789468	0.418844432706349	7.08892178382568	0.308019983826628	5.41754928350121	0.39110914744517	11.2233514013502	0.313227729548568
7.59349501561917	0.40978014479976	8.48416704594379	0.424712402463251	7.10334773418816	0.30940775097779	5.42155783962628	0.394848631921997	11.2280085197456	0.313652522952526
7.59469984267948	0.411321705323933	8.48439674361637	0.424908902742445	7.1083616161014	0.309890721835538	5.42238444329774	0.395620969076148	11.2328275320545	0.314092343576281
7.5952692362384	0.412050715219542	8.48602137981895	0.426299265992401	7.10885603152145	0.309938365052443	5.42910499212747	0.401915279925339	11.2348617472092	0.314278081236744
7.59546136516872	0.412296771693376	8.49115768623285	0.430700865286414	7.10926768703959	0.309978035734946	5.42918278500305	0.40198829152435	11.240432569801	0.314786975855222
7.59643844791223	0.413548637609129	8.49250726017119	0.431858846483196	7.11522088015384	0.310551984014309	5.42931904157474	0.402116181786393	11.2761600676023	0.318059015061538
7.59702059248316	0.414294916455133	8.49260640805458	0.431943942019574	7.13895694377794	0.31284495897963	5.43707287478211	0.409410783855258	11.2902959376399	0.319357573554391
7.59752137314449	0.414937138804924	8.49461577373838	0.433669193050469	7.14245894974676	0.313183879961866	5.43930510390917	0.411516753926568	11.2931504049847	0.319620062266106
7.60079885793043	0.419145862669617	8.49634249820049	0.435152778563208	7.15923802768725	0.314809930350533	5.44032756293766	0.412482236597286	11.2933913254522	0.319642220766277
7.60134146207918	0.419843545372175	8.49740056066072	0.436062308588054	7.16041965550882	0.314924577127242	5.44053622273885	0.412679334148825	11.30457592934	0.320671624941115
7.60267669920377	0.421561467602236	8.4979838369469	0.436563848581979	7.17214793509041	0.316063472503195	5.44100174976691	0.413119144700048	11.3060155618933	0.320804225732481
7.60439882714507	0.423779367229939	8.49890486146439	0.437356014495286	7.19587701709095	0.318373064210509	5.44424035417655	0.416181832524935	11.3124109698399	0.321393566251645
7.60606172295894	0.425923277414798	8.49898156723902	0.43742199990095	7.2105254418948	0.319802359851554	5.44564758911328	0.417514227897008	11.3408900222275	0.324023373202982
7.60608183712524	0.425949223408351	8.50406342677862	0.441797410706058	7.21896841545142	0.320627387867728	5.44670798500614	0.418518856759689	11.3450306857777	0.324406465900556
7.60615123119453	0.42603873979857	8.50410236066744	0.441830960377255	7.22593629180022	0.321308941075669	5.44708009296753	0.418871521648379	11.3462172273308	0.324516278585773
7.60686404044022	0.426958463436474	8.50479930243219	0.442431591535484	7.24146891226567	0.322830407726279	5.44762061403836	0.419383915945007	11.3657858811381	0.326329523897189
7.60969476040563	0.43061475862828	8.50878617921951	0.445870023533979	7.24430554988619	0.323108586364463	5.45095973400985	0.422552279350053	11.387442721464	0.328341056365402
7.61001015908977	0.431022517396793	8.50999439647233	0.446912851872632	7.24443835755033	0.323121612750742	5.45112450900234	0.422708759628636	11.4004562899952	0.32955218650248
7.61022825339855	0.431304520599429	8.5113021915651	0.448042040788794	7.2470920245188	0.323381942058429	5.45297542200233	0.42446733071959	11.4020659214484	0.329702114268695
7.61554935210257	0.438195388091362	8.51136997869605	0.448100581759362	7.25305415651858	0.323967152808755	5.45674278613693	0.428051353672226	11.4096595150003	0.330409781943517
7.61994311378965	0.443899600858073	8.51238385304605	0.448976297892316	7.25820279123815	0.324472865432292	5.46420896577247	0.435171472746165	11.4160608952468	0.331006815618401
7.62036783037618	0.444451626265965	8.51505756668868	0.451286852360098	7.26772079679303	0.325408601549703	5.46441372142041	0.435367045305364	11.4310811535462	0.332409387037295
7.62126906390632	0.445623360264389	8.51584780423756	0.451970074996405	7.27161001898446	0.325791276960701	5.46512110963688	0.436042829228013	11.4503629849343	0.334213341695493
7.62408697470837	0.449290071279994	8.5210026994089	0.456430288543776	7.30614818783055	0.329197635823582	5.46970081029251	0.440422353581578	11.477576874369	0.336765919518168
7.62735740395063	0.453551021553639	8.52209561052556	0.457376642319689	7.31120068706101	0.329697142931867	5.47345702027227	0.444019854671033	11.4966994334393	0.338564073535873
7.63011904276342	0.457153271979475	8.5239419324177	0.458975922277834	7.34957583065033	0.333500905455763	5.47432584552804	0.444852638372959	11.526274652237	0.341352373482726
7.63584397141597	0.464631692980506	8.52439987115191	0.459372691604044	7.38138155937121	0.336666551270985	5.47457047438204	0.445087163352341	11.527342283867	0.341453191200135
7.63598101926019	0.464810881194064	8.52494596435595	0.459845892992812	7.39784900989099	0.338310144540357	5.47700475439065	0.447421934714476	11.5293543940685	0.341643227897205
7.63667327269098	0.465716101565586	8.52658938427713	0.461270291840768	7.41004873553387	0.339529774070201	5.47875006592682	0.449097028242293	11.5303999912455	0.341741996709229
7.63962955560416	0.46958380376648	8.53064874771674	0.464790749632541	7.42985063180935	0.341512984548434	5.47911712019047	0.449449431566509	11.5361415403346	0.342284545728575
7.64466347712326	0.4761760914081	8.5343803164125	0.468029369161045	7.43900641927197	0.342431445599274	5.48150829290081	0.451746124462319	11.5459236644369	0.343209659499256
7.64790033609027	0.48041855584468	8.53643066794384	0.469809779341622	7.4391851538797	0.342449384624669	5.48358301932477	0.453740186672823	11.5776131216627	0.346213024463956
7.6530494326692	0.48717171693998	8.53776047403933	0.470964833333505	7.44482684801039	0.343015806044946	5.48381387107091	0.45396213608606	11.5826909914659	0.346695185393421
7.65422500094868	0.488714088275107	8.53790151862215	0.471087357504979	7.46568837358114	0.345113343093364	5.48617062366072	0.456228815841571	11.6038745211371	0.34870930543354
7.65439515940366	0.488937354425092	8.53878024855473	0.471850763548144	7.4688802764406	0.345434697384852	5.48648718548753	0.456533389173164	11.6601615566323	0.354081674821743
7.65708783865027	0.492470853983429	8.54045972566138	0.473310112673626	7.47228586369962	0.345777687873222	5.48969561204797	0.459621720213983	11.7066140694111	0.358537418372501
7.65863594044131	0.494502653816993	8.54497665823977	0.477236736890715	7.49245445949957	0.34781153583012	5.49175202551326	0.461602453417112	11.7119045687218	0.359046122393054
7.66380465164281	0.501287042934906	8.5461431305759	0.478251139982455	7.50022471779064	0.348596280678255	5.49185251162817	0.461699266251034	11.7280684487624	0.360601893895629
7.6655860999734	0.503625363987618	8.5467134705939	0.478747178308715	7.51205145830269	0.349791947030073	5.49251651196482	0.462339050761736	11.7425447478944	0.361997198153979
7.66769504954708	0.506393394333932	8.54740136446789	0.479345499758059	7.52178946904179	0.350777565978364	5.49530113963383	0.465023166389808	11.7530475541222	0.363010666169272
7.66798636681149	0.50677573175712	8.54773816219122	0.47963845924321	7.52323884050542	0.350924348146959	5.50541042648747	0.474780041925824	11.76875505938	0.364528151393993
7.67076378067025	0.51042056754332	8.54935532383115	0.481045278437548	7.52540356542676	0.351143617719119	5.50795387076935	0.477237436473406	11.7874752421811	0.366339463034636
7.67110800156459	0.510872238623782	8.55699568380377	0.487694764007535	7.55208621293224	0.353850410244298	5.50891258344505	0.478163943735354	11.7922786924579	0.366804713550588
7.6715554798194	0.511459378409789	8.56034823959172	0.490613718143065	7.55510842605319	0.354157464751127	5.5136188487916	0.482713731825422	11.8214391181445	0.369633299802321
7.67481430819428	0.515734483817442	8.56685733926463	0.496282261196656	7.57456507642941	0.35613650852225	5.51376635082566	0.48285636909924	11.8508652942931	0.37249483331079
7.67592321921292	0.51718882493386	8.5700066841689	0.499025253693155	7.61925882288859	0.360697182805377	5.51425217084533	0.483326181720021	11.8535552504692	0.372756770932454
7.6775493016995	0.519321019484755	8.57055372825455	0.499501722332938	7.62452297167729	0.361235672627402	5.51730707363297	0.486280931985121	11.8746586483164	0.374813771953298
7.67793917181082	0.519832155363471	8.57144166697632	0.500275107201552	7.6532358840444	0.364177642595519	5.52167682690716	0.490508695489707	11.8772210950932	0.375063784049127
7.68138562349623	0.524349082915963	8.5726669507783	0.501342313625671	7.67599985530553	0.366515786110247	5.52570920033387	0.494410998998627	11.8809545103732	0.375428138824642
7.68188445916665	0.525002612704334	8.57304108792287	0.501668180702126	7.67683892709998	0.366602064601717	5.52780700181138	0.496441368061166	11.8896849615622	0.376280602111922
7.68306820765685	0.526553181470313	8.57337184895116	0.501956267000612	7.72581712796648	0.371649850864428	5.53001233818186	0.498575913804504	11.8900947370013	0.376320628489239
7.68382200372884	0.527540355925382	8.57341499127209	0.501993843034872	7.73108745507957	0.372194356019175	5.53042470696122	0.498975052033735	11.9006271938768	0.377349881676809
7.6877008289048	0.532617275026377	8.57615457003874	0.504379906809719	7.75176543677462	0.374333166627623	5.53120104753382	0.49972648675288	11.9567779298095	0.382851594395156
7.68823129796172	0.533311202034465	8.57662469637777	0.50478935470769	7.79780362755388	0.379108915767239	5.53940863592173	0.507670305782275	11.9622083402136	0.383384947843529
7.68902443392185	0.53434854424247	8.57990480082699	0.50764593710292	7.80673307129286	0.380037373426553	5.53980629798633	0.508055136206188	11.9856054452253	0.385685435470392
7.68996418738884	0.535577344843562	8.58567814548384	0.512672793918916	7.80838802788842	0.380209527161362	5.54151639467046	0.509709962067656	11.9918082568903	0.386295996883952
7.6910404616709	0.536984239572535	8.58630958817435	0.51322248394886	7.83857004794631	0.383353286003419	5.54264237153097	0.510799457553555	12.012191146395	0.388304322020441
7.69128471180019	0.537303457085714	8.58732085295808	0.514102767874429	7.8445659540922	0.383978742440108	5.54270713396265	0.510862119325379	12.0299411230728	0.390055664550706
7.69296486839441	0.539498640214047	8.58804437905353	0.514732539630939	7.84553811353443	0.384080180720569	5.54354150870547	0.511669405432702	12.0393817707995	0.390988060345
7.69425466465683	0.541182991147515	8.59273001355311	0.518810051891609	7.84849032314359	0.384388272528544	5.54490625249939	0.512989737179936	12.0481855433716	0.39185812094002
7.69504865555896	0.542219501961203	8.59423572032108	0.520119944261799	7.86812631891469	0.386439329862653	5.54582487960538	0.513878390670743	12.0594522283678	0.392972375493494
7.69592003849308	0.543356713096473	8.59443322093851	0.520291744473839	7.88130258374009	0.387817427721322	5.54628645003395	0.514324874916907	12.0625637627217	0.393280255581076
7.69750418835479	0.54542321545846	8.5948393562572	0.520645018242058	7.90086082883264	0.389865616358018	5.54637088317675	0.514406546481245	12.120592559871	0.399034122377908
7.69924389597394	0.547691223162521	8.59489698580945	0.520695145569463	7.96679639139787	0.396792805994824	5.5486637960964	0.516624222011446	12.1218931424112	0.399163338931416
7.70025582530744	0.549009736196843	8.59732772729546	0.522809144765549	7.98165645271343	0.39835859736545	5.55180954094661	0.519665895043101	12.1269606569192	0.399666916107375
7.70130180546639	0.550372048097365	8.59749678374669	0.522956148819966	8.00293657835072	0.400603711829238	5.55418180111598	0.521958925388586	12.1292660940094	0.399896071000299
7.7025736645651	0.552027749594543	8.61079826956541	0.534511125827929	8.00586909173835	0.40091335984111	5.55435342517262	0.522124790186577	12.1567807741299	0.402633603967309
7.70412482251177	0.554045812302826	8.61200744379752	0.535560239206383	8.06645205688006	0.407324052520514	5.56654037784666	0.533891274332482	12.161076222115	0.403061408155654
7.70521429944082	0.55546239276375	8.61264075539484	0.536109619888592	8.07141344220478	0.407850176722059	5.56699669316258	0.534331335647813	12.2498416008182	0.411927234339488
7.70578539218468	0.556204668127473	8.61373978171801	0.537062831494993	8.11718740254735	0.412711944807699	5.56792841752048	0.53522974094978	12.2782643550892	0.414775842313867
7.70609821128375	0.556611170022406	8.61474628698851	0.537935610876888	8.12025605825363	0.413038362812893	5.56801330201452	0.535311581064294	12.2952949052283	0.416484851492881
7.71079526539805	0.562707495104644	8.61513855288027	0.538275710471447	8.12392133865992	0.413428323565063	5.56895577452312	0.53622015068007	12.3253645777142	0.419506170079003
7.71189857926634	0.564137388848563	8.62722714258607	0.548741751232683	8.13045412154821	0.414123578507094	5.56958516685776	0.536826797446184	12.3444810114248	0.421429419396012
7.7127459914744	0.565235066320382	8.64236877799134	0.561802555695806	8.13803286449447	0.414930487514185	5.57199969859458	0.5391532639146	12.3756571629178	0.424569967181335
7.71299900969235	0.565562711056218	8.64256090762979	0.561967881067032	8.14555163843003	0.415731366426691	5.57469608000196	0.541749713536731	12.3955204865544	0.426573424191961
7.71349732946877	0.566207875999646	8.64280388367487	0.562176943702631	8.15560090869079	0.416802332986499	5.5777364315592	0.544675244301378	12.4383270482853	0.430897365596746
7.71503499883356	0.568197547698277	8.64434620734167	0.563503590271943	8.15593170273507	0.41683759677429	5.57816898880737	0.545091272702815	12.4607000696539	0.433160625578555
7.71540045790473	0.568670182131572	8.64522498018744	0.564259158014964	8.1681068343259	0.418135971131055	5.57963069494514	0.546496755675287	12.5072082518862	0.4378723418381
7.71594446597934	0.569373544980801	8.64832364181935	0.566921493959107	8.18358452900816	0.419787822824754	5.5811675419152	0.54797386114294	12.5119874403787	0.438357029773556
7.71656743105042	0.570178723128434	8.64882923130019	0.56735560610944	8.19786841667008	0.421313521539988	5.59038454008169	0.556817935559002	12.5461474554314	0.441824064466042
7.71735260465799	0.571193138672157	8.64977400311303	0.568166593260985	8.2147987957851	0.423123428300704	5.59044480998759	0.556875678773408	12.592842930341	0.446570540138746
7.7200014945826	0.574611901284718	8.65418238182145	0.571946872007945	8.22657568609627	0.424383372022547	5.59270883332819	0.559043902025063	12.6176851996754	0.449098860650336
7.72119351387698	0.576148556392794	8.65497189945374	0.572623213999426	8.24264624909844	0.426103916762191	5.59356618277753	0.559864515324179	12.6304163451073	0.450395380319544
7.72205979997452	0.577264577878898	8.65612546132897	0.573611031102999	8.25138941601231	0.427040570013026	5.59807648460308	0.56417724285571	12.6363776712281	0.451002655202523
7.72568561744957	0.581928829872575	8.65665308202444	0.574062689325627	8.26801897730778	0.428823222141105	5.59998336825922	0.565998333006278	12.6451485715326	0.451896346996767
7.72737331324741	0.584096000110122	8.65704111457611	0.574394794195964	8.36117290882486	0.438834973239646	5.60164947572314	0.567588335388042	12.6799362644731	0.455443320909909
7.72760947157267	0.584399048760823	8.66578786679364	0.581866426625044	8.36870824788047	0.439646639046967	5.60377358031568	0.569613824853882	12.7002426716151	0.45751543565442
7.72849023503615	0.585528838754184	8.67091991200193	0.586236779088379	8.37456002983405	0.440277136457156	5.60706893838771	0.572752549663511	12.7113462153038	0.458648960261829
7.72936993385411	0.586656557204139	8.67446413983988	0.589248787229388	8.48807121214881	0.452535392440386	5.60999033086545	0.575531244667829	12.7357185935135	0.461138223560173
7.73431328748209	0.592980080518288	8.67640364545488	0.59089483338985	8.54739975440439	0.458961185914415	5.61095560406528	0.576448551026372	12.7901833034405	0.466706317576757
7.73615006336581	0.595323610251621	8.67717396629293	0.591548157087229	8.57619191640785	0.462083600188659	5.61115563317768	0.576638588550275	12.794404645868	0.467138164694229
7.73637760140595	0.595613688420268	8.67748159205562	0.591808989355277	8.57712366888031	0.46218468574225	5.61130202945805	0.576777660942597	12.8352111522454	0.471314625912645
7.73765506611155	0.597241291467048	8.67817351220693	0.592395511520977	8.59423765470597	0.464041804830849	5.61174899605324	0.577202207511381	12.8718010867469	0.475062227799826
7.74228927002562	0.603131348420791	8.67818270297599	0.592403300899061	8.61520304925542	0.466317922493245	5.61230346063821	0.577728735291137	12.9069092563787	0.478660144454429
7.74408317239404	0.605405170242332	8.67895911783955	0.593061197305914	8.63237697175426	0.468183241797275	5.6145878049366	0.579896507767624	12.9161551929631	0.479607977713995
7.7453122621181	0.60696101073088	8.6827101639788	0.596235922796431	8.65111155906261	0.470218865846693	5.61673479348163	0.581931727912216	12.9662442105248	0.484744645490746
7.74983953510867	0.612676946621207	8.68630212465389	0.5992700771301	8.68950722067345	0.474393157181882	5.62084129790262	0.585818305529373	12.9984962344191	0.488053509723669
7.75047890811418	0.613482257442204	8.69184349254659	0.603939123996058	8.72460287365291	0.478211151217194	5.62963321141147	0.59411069679044	13.0515857774765	0.493501862948467
7.75060464687195	0.613640572071442	8.69220990677377	0.604247340423909	8.78636967501618	0.484935295948571	5.63006373987366	0.594515714150735	13.055475335761	0.493901091732194
7.75105036548483	0.614201613059217	8.69462672896643	0.606278656027686	8.78927068166728	0.485251229759379	5.63019026287967	0.594634720778771	13.0754225439796	0.495948583719928
7.75111773963346	0.614286398414303	8.69547289384365	0.606989169522539	8.81541267232668	0.48809861413634	5.6358538402208	0.599952722675287	13.0778472877077	0.496197481204795
7.75221560178395	0.615667204170934	8.69566170185123	0.607147660582519	8.81695123362768	0.488266214484481	5.63904154844983	0.602937861707378	13.0906750224436	0.49751425749114
7.75520046790636	0.619413877126501	8.69623987412114	0.607632885007253	8.83443516558374	0.490170932874485	5.63956578306913	0.603428210943257	13.0954050733061	0.497999808243169
7.75543445546859	0.619707115962747	8.69751709137968	0.608704180959605	8.86454148532327	0.49345124864901	5.64230838082824	0.605990850696467	13.1405352626951	0.502632573453737
7.7554642126938	0.619744403505848	8.69770652978196	0.608863006879322	8.88948207325964	0.49616906313584	5.64381699365663	0.607398528310989	13.1820118836486	0.506889989431199
7.75573339616422	0.62008165553174	8.69974902782131	0.610574287311382	8.90681220859664	0.498057667082234	5.64800633717713	0.611300165064153	13.2484785140871	0.51371069472591
7.75591246967063	0.620305960887748	8.7060296806403	0.615822897721281	8.92521586386538	0.500063307815011	5.64838641400338	0.611653591422214	13.2583649124823	0.514724927828503
7.75596902991754	0.620376799176462	8.70636985796455	0.616106580989816	8.93035096098544	0.500622935484243	5.64971184971233	0.612885364431012	13.2878622786758	0.517750433502315
7.75786369022142	0.622747398359222	8.70682376942946	0.616485013399902	8.9320893779657	0.500812389563958	5.64986769125785	0.613030118949529	13.3052304462232	0.519531396532668
7.7583554668397	0.623361958003219	8.70937601669668	0.618610779931522	8.9364194923086	0.501284288016431	5.65532258261767	0.618086893099705	13.3222245105317	0.521273621312938
7.75842071661285	0.623443475391345	8.71178824356645	0.620616640825271	8.96861929537688	0.504793341027627	5.65763892226141	0.620228154587992	13.3367517738692	0.522762629709523
7.75855114042136	0.623606399046542	8.71194229519134	0.620744631187258	8.97389358843128	0.505368091995031	5.66076820659323	0.623115059684967	13.3666162522774	0.525822643682662
7.75981230041159	0.62518068309811	8.71426458522091	0.622672443291769	8.97785862620381	0.505800163348688	5.66517118089217	0.627165338263612	13.4536555353682	0.534731638302228
7.76023207212486	0.625704215916654	8.71462145863813	0.622968426644765	8.98683253848492	0.506778027342669	5.66840017440777	0.630126795423023	13.5005152216649	0.53952109609661
7.76060393830034	0.626167808174059	8.71489007243385	0.623191161671487	9.02681947124509	0.511134722572692	5.66960795134244	0.631232533438245	13.519372011881	0.541446842913338
7.76128043201927	0.627010700395641	8.71797633154227	0.625747334393578	9.10989510237813	0.520181217321973	5.67870943106554	0.639529583603708	13.5313217046117	0.542666702996536
7.76342428124846	0.629677845186384	8.72378125015766	0.630540190626628	9.1103367547933	0.520229287290328	5.67954748170746	0.640290339623604	13.5368451270049	0.54323041522867
7.76348697819933	0.629755752898385	8.72541250057281	0.631883432958209	9.14663227832484	0.524178664655249	5.68031508805657	0.640986661196534	13.5606307743913	0.545656934878326
7.76351615570427	0.629792007275045	8.72847449848494	0.634400454272384	9.18387245038213	0.528228359878821	5.68410431907944	0.644417100983059	13.5710725230531	0.546721629110997
7.76377847284661	0.630117896434038	8.73177271409542	0.637105189157706	9.20102843517084	0.530093037250363	5.68432466607181	0.644616227695121	13.5808965461331	0.547723030480718
7.76511607317927	0.63177820421226	8.73650334606719	0.640972650429978	9.22821683163295	0.533046766155028	5.68615690988309	0.646270485864819	13.5898160783653	0.548631970833613
7.7690038511016	0.636589887357386	8.73953277610847	0.64344177975749	9.24634610863278	0.53501531775246	5.68779875645687	0.647750500486755	13.5903409401342	0.548685448707739
7.76938335803002	0.637058443381974	8.74162283648296	0.645141787793126	9.28942081206002	0.539689022995033	5.6886629600175	0.648528625823491	13.6134533798642	0.551039472550215
7.77140521060002	0.639551239569687	8.74416498830751	0.647205625173686	9.35895785526958	0.547222119573325	5.69367547348773	0.653029515315641	13.7371439842332	0.563604952524897
7.7714838369738	0.639648061220355	8.74541679163256	0.648220312439348	9.36048492865566	0.547387370195556	5.69710164153433	0.656093647137851	13.7703658223152	0.566969525077696
7.77355130106496	0.642190735831063	8.7461993350981	0.648854091522047	9.3838474928617	0.549914485102931	5.69800452346258	0.656899429497812	13.7899857633039	0.568954291347781
7.77491192509376	0.643860674293656	8.75087409107001	0.652631486610573	9.39742071744105	0.551381770556535	5.69945173691013	0.658189515415431	13.7994547555434	0.569911561450469
7.77506559417328	0.644049104792061	8.75147229692052	0.653113778810183	9.4040215681228	0.552095079523924	5.69997842543818	0.658658562933017	13.8340605523191	0.573406507859592
7.77674327111786	0.646103990730647	8.75648305619541	0.657143805419784	9.44662233337348	0.556694503493034	5.70634275271274	0.664306826088124	13.8348896384347	0.573490170314716
7.78047000860342	0.650653373990661	8.77269393359631	0.670057816332963	9.45015709282508	0.557075802222744	5.70696362566823	0.664855886630394	13.8520549727775	0.575221562917943
7.78135631730171	0.651732178725189	8.77283222823293	0.670167145393666	9.45079444989177	0.557144549077796	5.70733459506022	0.665183780422649	13.8668576930696	0.576713485765768
7.78143069081822	0.651822649653808	8.77296633782005	0.67027315207385	9.50016059493196	0.562463914435071	5.71124567789401	0.668633020719523	13.8759476786913	0.57762909541576
7.78368539098237	0.654561235211274	8.77444245565529	0.671439041403291	9.50353713558801	0.562827346911222	5.71281911148638	0.670016650291121	13.905381850324	0.580591018161048
7.78585201542673	0.657185243910195	8.77475944121942	0.671689190605355	9.59299626584964	0.572436003978322	5.71415890199947	0.671192991561118	13.9899118239675	0.589071248704743
7.79236216394026	0.665023777956046	8.7758352941522	0.672537625711339	9.62192609176806	0.575534422415927	5.71527376402739	0.672170554241842	13.9987338466407	0.589953971100401
7.79299126080294	0.665777513393589	8.77875605021568	0.674836481763463	9.62799117451243	0.576183415167553	5.71645350665571	0.67320372387856	13.9994861470397	0.590029224472836
7.79416929502731	0.667187144931863	8.77946912903691	0.675396723836638	9.63034914418023	0.576435673485409	5.7198487953612	0.676169752039372	14.0023630179565	0.590316970182861
7.79794810057989	0.671692843486406	8.78029092711911	0.676041891011496	9.64406014965926	0.577901868872625	5.72652457071305	0.681968872073936	14.0148315424081	0.591563512550961
7.79832553707221	0.672141528742835	8.78080711018372	0.676446859618457	9.64621009326132	0.578131677160585	5.73307851424446	0.687619093937932	14.0157414897803	0.59165444855903
7.79870026128709	0.672586744044038	8.7853155614274	0.679975016905863	9.70151017679049	0.584033366392396	5.73330041524696	0.687809637045843	14.1005620446751	0.600108723452132
7.80157643425263	0.675995758849526	8.78670642255298	0.681060198653883	9.72265547293395	0.586285094341223	5.73566936085289	0.689840677060742	14.122910026802	0.602328587829987
7.80392370884409	0.67876701121876	8.7872937333431	0.681517967052848	9.72985142635164	0.587050736969027	5.74054042091336	0.693998729986173	14.1278428958904	0.602818135038122
7.80606888453463	0.681290989430529	8.78809778168142	0.682144218268079	9.7641430232759	0.590694735069605	5.74429196617685	0.697184221193518	14.1286043185496	0.602893685646576
7.80691761880183	0.682287287258433	8.78923834269583	0.683031676700275	9.77573485115653	0.591924787778614	5.74838137936403	0.700639580960971	14.1644536903006	0.60644634917353
7.81206453588006	0.688300612220143	8.79099423749591	0.684395862475875	9.82628740667563	0.597278375821474	5.75043305772994	0.702366388459338	14.180186504577	0.608002692637117
7.81218007323706	0.688435032015352	8.79227725481399	0.685391076376163	9.82903010421236	0.59756832015747	5.75384142023933	0.705224962166149	14.1889034699108	0.608864262846539
7.81351760818967	0.689989330609318	8.79561739687284	0.687975641717776	9.85306212257735	0.600106553464419	5.75577583628303	0.70684169424262	14.1893170766517	0.608905129806102
7.81607060987711	0.692946653380387	8.7962851140018	0.688491211327167	9.85756154333019	0.600581310724534	5.75615732154152	0.707160043162771	14.1986594640041	0.609827895570152
7.81785858804662	0.695010362307305	8.79862509100257	0.690295075396096	9.86333818649741	0.601190616268578	5.76028116052544	0.710591091266753	14.2048511184884	0.610439116891587
7.81794699242618	0.695112239858118	8.79966810956849	0.6910976567733	9.91488121294669	0.606616165121327	5.76118371341531	0.711339491877188	14.2240356503463	0.612331215514616
7.8215115669967	0.699207401351105	8.80234500851276	0.693153296953341	9.92915969917323	0.608115548695536	5.76231789090057	0.712278662066846	14.2403030266207	0.613933520622513
7.82455441774629	0.702683416675701	8.80383589033811	0.694295550452251	9.9495348597347	0.610252361203943	5.7653676331586	0.714796853575762	14.2691830488865	0.616773348658545
7.82543967961335	0.703691242599998	8.80389228832149	0.694338723318442	9.96355764241664	0.611721048907271	5.76648697250899	0.71571845716123	14.298732775181	0.619672548192376
7.82560843955141	0.703883189343833	8.80768354153779	0.697234722761802	9.97068028328503	0.612466434659423	5.76739862281294	0.716468007386122	14.3055534756268	0.620340797379382
7.82680059417853	0.705237512127956	8.80974942353951	0.698807583768343	9.98024792218971	0.613467037402602	5.7740167643553	0.721880796219716	14.3741056795648	0.627036849754368
7.82683192577881	0.705273067201686	8.811127014617	0.69985436379453	9.99991239824441	0.615521213621573	5.77560698577784	0.723173842335007	14.396356230899	0.629202129006661
7.82684577790332	0.705288785950462	8.81429792498218	0.702257545173002	10.0228627836741	0.617914540552541	5.77632101286118	0.723753474992396	14.4060947339329	0.630148535760108
7.82707685245668	0.705550941605878	8.81449269308057	0.702404870190677	10.0371485943683	0.619402037133911	5.777612744461	0.72480056079201	14.4258853807687	0.632069397218223
7.8307240920481	0.709674425354165	8.81647288574812	0.703900819982276	10.0382881660756	0.619520618303485	5.77821386419081	0.725287165112687	14.4514178611436	0.634542678773172
7.83090884678192	0.709882583164627	8.8167625721197	0.70411937583337	10.0524494843359	0.620993271826318	5.78322042062838	0.729323395757731	14.4984491463112	0.639083827945634
7.83221761521561	0.711355128232594	8.81761576450361	0.70476264178688	10.0546083484841	0.62121762126259	5.78796536021343	0.733121183816342	14.5069035079691	0.639898093297932
7.83617169453885	0.715782494098617	8.81801199083787	0.70506115829502	10.0755922219997	0.623396129836423	5.79476505148354	0.738516231787403	14.5137945390005	0.640561320501432
7.838480672302	0.718352741988865	8.8222584645935	0.708251677477807	10.1071369254412	0.626663643790349	5.79620846378593	0.739654224155464	14.5140424901139	0.640585176677047
7.84229287231148	0.722571617679257	8.82387263675918	0.709460226636456	10.154348371635	0.631536938972771	5.79623503168555	0.739675146461448	14.5345311105021	0.642554551517524
7.8444302327499	0.724923393336186	8.82456537057297	0.709978164944705	10.1882656110913	0.635025007015718	5.79736823468849	0.740566740319929	14.5905409635671	0.647918765888709
7.84591575689202	0.726552137435039	8.82514702173541	0.710412715184302	10.2437032560914	0.640702145625513	5.79922220437778	0.742022018188129	14.6361948275248	0.652269546672721
7.84711174006638	0.727859947329973	8.82849950442926	0.71291136902147	10.2573131493109	0.642091198184395	5.80767764138156	0.748605039764888	14.6508396000192	0.653660978803839
7.84814584019125	0.728988225740353	8.83365988925787	0.716737404495459	10.3500311462351	0.651503329781862	5.80917054126017	0.749758052265783	14.7424011686915	0.662312843479507
7.85018576533285	0.731207068456018	8.84571829977722	0.725581239119464	10.4052337469066	0.65706359898772	5.81177528637926	0.751763043066018	14.7565960208101	0.66364664218805
7.85147034322827	0.732599616691229	8.8518800850824	0.730047176200496	10.4339132397524	0.659939055291841	5.81194690714694	0.751894845922184	14.7617676619456	0.664132077628571
7.85335525183913	0.734636345437598	8.858449847039	0.73476839797634	10.4632858413371	0.662874390698718	5.81224855188112	0.752126415252923	14.7876817040763	0.666560360408306
7.85657801071971	0.738100347800626	8.85890261154285	0.735092216792257	10.4735366333796	0.663896479723769	5.81261886432286	0.752410542198575	14.8354810976835	0.67102109384314
7.85848514876181	0.740139270332845	8.85895953859198	0.735132917000021	10.4739673054385	0.663939394854898	5.81349660716937	0.753083306098301	14.8400636507968	0.671447482755768
7.85963241004367	0.741361851417183	8.8595989825725	0.735589871404271	10.5020760374209	0.666735699054774	5.81503185032336	0.754257668444884	14.8844345560445	0.675564413771524
7.86336491568225	0.745318699106514	8.86416305687334	0.738839719426639	10.5286927547502	0.669375062561268	5.81739366834979	0.756058436218412	14.8854203114887	0.675655635749729
7.86350538626438	0.745466991251131	8.86652377975541	0.740512580032656	10.5481486886558	0.671299044247805	5.81784052812355	0.75639834163878	14.9031989572825	0.677299060725574
7.86354661204935	0.745510503947193	8.86813190730557	0.741648957684359	10.6081517099371	0.6772039780864	5.81928581174217	0.757495947995775	14.9944795650882	0.685681865909277
7.86766227020402	0.749834776989661	8.87345775396262	0.745393953200979	10.6259515011674	0.678947193905086	5.81952094032254	0.757674260387227	14.9972708981205	0.685936735478194
7.87120633507679	0.753527019093089	8.87367726015222	0.745547691774036	10.6653121327384	0.682787945038111	5.82336394340316	0.760578549513119	15.0663429284372	0.692215037403221
7.87386305145836	0.756275546062553	8.88709782814565	0.754854065179994	10.6931180236474	0.685489416227485	5.82510156642974	0.761885463395668	15.1200442195503	0.697057748719206
7.8739122742947	0.75632631334038	8.8910966281231	0.75759117698119	10.7492843168746	0.690915928484193	5.82610596324134	0.762639111066473	15.1283824227	0.697806608294824
7.87453899068351	0.756972194486861	8.90050570020412	0.763965694459714	10.7648191840309	0.692409573296712	5.82762932735426	0.763779661036603	15.1404257872101	0.69888676155446
7.87655665301012	0.759045252294188	8.90059326808957	0.764024583498017	10.7903753387723	0.694859809295575	5.83389356175046	0.768437848662906	15.1982348815934	0.704047183373343
7.87788121087873	0.760400929189811	8.90446207433007	0.766618242720606	10.8107958851834	0.696811409844911	5.83876476210356	0.772024476529831	15.2088589387642	0.704991122574779
7.87929173066829	0.761839997976185	8.90929128166833	0.769833445246787	10.8378855126745	0.699391725864898	5.8393695222328	0.772467565789626	15.2469318381022	0.708362423830744
7.88210140067944	0.764692369751776	8.91714465250098	0.775008776174411	10.8422001667714	0.699801784364196	5.84084300688858	0.773545110077205	15.27199731833	0.710572085973721
7.88537774010407	0.767994548737479	8.92091490956559	0.777469733866187	10.873226454714	0.702742999236005	5.84836347559526	0.778999649149169	15.2790516612298	0.711192544576081
7.88631196926824	0.768931396404687	8.92254130811689	0.778526575063289	10.9155632293973	0.706735031584985	5.85010132224511	0.780249315424332	15.2965894201323	0.712732343485524
7.88835704694911	0.770974817548887	8.92967744654571	0.783129614127074	10.9257301623279	0.707689982019761	5.85490840950638	0.783684829930657	15.2992627044146	0.712966713697998
7.89074497495066	0.773347928225344	8.92991103981987	0.783279348534338	10.9327920663993	0.70835243381071	5.8552640709952	0.783937771710408	15.3246380390513	0.71518687917299
7.89215330975224	0.774740992562177	8.93109963051711	0.784040314201466	11.071058504362	0.721179442305293	5.85884128655118	0.786472296726821	15.3726791534565	0.719367558253224
7.89368319409718	0.77624877825894	8.9320160424952	0.78462596583469	11.1146334277084	0.725164238171967	5.85902115014668	0.786599274354956	15.4627085024575	0.727121286961312
7.89973328113274	0.782154950635416	8.93337441967625	0.785492366877326	11.1298805043594	0.7265518780725	5.86012234822841	0.787375722787044	15.4900397790282	0.729453976687439
7.90163636912625	0.783994011436625	8.93715309514246	0.787891798980205	11.1824732776373	0.731311578371556	5.86130953792693	0.788210952459004	15.6528481816737	0.74313976194847
7.90181312696294	0.784164364779032	8.93984962971088	0.789594442538094	11.1956031579787	0.732493319661767	5.86518784849976	0.790926065465282	15.6578321541314	0.743552961733445
7.90360000554768	0.78588212182137	8.94135674300553	0.790542557044128	11.2717995579702	0.739299155941324	5.87180245274049	0.795509206578509	15.6815550107823	0.745514964332002
7.90362604463582	0.785907094690525	8.94518003594519	0.792936458485694	11.3549499618108	0.746623109503479	5.87478492845275	0.797555999190887	15.8065517244693	0.755721519125979
7.90474119602027	0.786974992458206	8.94598336743616	0.79343738757163	11.4677089056767	0.756379507869397	5.87925514602876	0.800600746796934	15.8245460550473	0.757172452688684
7.90546052378235	0.787662187300908	8.946459257943	0.793733797186978	11.5105830693553	0.760035226054276	5.88116136259188	0.801890676561862	15.8761457445016	0.761307094016617
7.90616164302279	0.788330738647315	8.94777808914908	0.794553916048876	11.5397458910191	0.762504632905241	5.88518462236023	0.804596610645402	15.9820808216415	0.769673536559908
7.90775703908717	0.789847427036307	8.95131473821547	0.796743610674108	11.584639504157	0.766278650755967	5.88739909108202	0.806076374628359	16.0504674405141	0.774986214792456
7.9081486716603	0.79021876052795	8.9539497073592	0.798365944057274	11.6372552531906	0.770659200667974	5.88782511476007	0.806360269139815	16.2494511831173	0.790043049382698
7.90980918910764	0.791788919282076	8.95592211106245	0.799575248438838	11.7752632747535	0.781927618322713	5.88893961182167	0.807101750309209	16.3648385619286	0.798496115903416
7.91411236097551	0.795825521652418	8.95819902912888	0.800965823471807	11.7916289348402	0.783242382763584	5.89091038592997	0.808408665559924	16.42070043951	0.802514120234283
7.91772649078595	0.799179480151764	8.96504760958617	0.805113260387217	11.8987193049229	0.791731810862194	5.89396831809305	0.810425759776254	16.4542711048653	0.804905298831873
7.92058809646143	0.8018114839369	8.96645541571454	0.805959256581425	12.0576682563425	0.803963985234123	5.89840458300936	0.813328712068335	16.5590151543771	0.81225217092152
7.92598268557898	0.806716257029122	8.96759101631995	0.806640042628353	12.1052009680051	0.807535549466497	5.89986680349928	0.814279480673333	16.5802683713213	0.813721772031868
7.92711332197698	0.807734765423174	8.96983200204677	0.807979218023804	12.1538768099749	0.811151482655192	5.89988858135803	0.814293618383812	16.6598563205555	0.819161477439135
7.92932507274147	0.809717656969471	8.97322773063707	0.809997600072168	12.1858602984147	0.81350446083574	5.90140313070929	0.815275192463837	16.6949769226167	0.821529921137145
7.93046047091513	0.810730672973795	8.97489932450475	0.810986368576792	12.200651613424	0.81458646881527	5.90654321450347	0.818582351276855	16.9100998630016	0.835607885561545
7.93725968897422	0.816727296175722	8.97648119818464	0.811919141723572	12.2232494507769	0.816231993688771	5.9090283994588	0.820167955367139	16.9171695876486	0.836057979513429
7.94106388302892	0.82003015334437	8.98184679988527	0.815061824209212	12.2259126656012	0.816425322099341	5.9107915185976	0.821287569916088	17.0354646021425	0.84347045730479
7.94503031417535	0.823433794017457	8.98316445409515	0.815828567277832	12.2821159066673	0.820475631917475	5.91508892082112	0.823998069281117	17.0457535712175	0.844104576490419
7.94509984096615	0.823493090398718	8.98402195676723	0.816326483761505	12.4370528434032	0.831347568325874	5.91675919122312	0.825044496798059	17.1032946040232	0.847619628964598
7.94555228926507	0.823878656173106	8.98496556599715	0.816873428469754	12.625220444088	0.843969464192641	5.9186422589706	0.826219497508123	17.1059159238243	0.847778496796534
7.95144475531846	0.828851312959455	8.99079559357049	0.820230119412684	12.6364440452272	0.844702119314501	5.91931165700966	0.826635977822818	17.1640445167978	0.851273181723974
7.95233509527077	0.829594787214758	8.99130049802812	0.820518992731312	12.8115067833383	0.855835725976747	5.92209295728226	0.828359611080239	17.2301791016984	0.855183474706788
7.95333132978364	0.830424232174077	8.99395033687732	0.822030268955889	12.9738491398307	0.865667752172944	5.92557667978204	0.830503049524816	17.2328787408118	0.855341609981704
7.95370478909601	0.830734498330588	8.99531197045333	0.822803715767371	13.0559714138279	0.870461850818538	5.92665958357839	0.831165815997003	17.2471232900004	0.856174078603737
7.95427159338236	0.831204696763446	9.00415930731202	0.827777419382723	13.0800228009552	0.871843192559106	5.92723374287421	0.831516540653038	17.4092902577942	0.865423453565428
7.95547739806309	0.83220218978064	9.01468069238092	0.833575051450329	13.0888962067099	0.872350225482226	5.93169435350114	0.834225327959627	17.4117941958903	0.865562992458241
7.95555853911088	0.832269176546054	9.01578938052044	0.834178550927813	13.0965541823218	0.87278668537168	5.93385628858914	0.835528015773178	17.4582119151817	0.868131767267862
7.96125947151905	0.836932503576519	9.01646443052185	0.834545311534934	13.097272777436	0.872827587748288	5.93509753856419	0.836272932305229	17.4704891787122	0.868805496143683
7.96344264238827	0.838695791225882	9.01785258923217	0.83529785995454	13.111013962158	0.873607974827056	5.94290434938428	0.84090777339066	17.5671546203693	0.874027084120954
7.96352282607846	0.838760315749899	9.02310872001662	0.838127183098348	13.3270037089949	0.885437570096437	5.94834169306314	0.844084597266954	17.6578384367699	0.878792190449378
7.96654649506362	0.841181197502066	9.02798662656931	0.840724410504986	13.3609849215968	0.887224487534248	5.95471245970752	0.847753217548328	17.6850243178845	0.880195686728837
7.97994469388456	0.851620275842395	9.04316859983512	0.848632399831832	13.3657671565103	0.887474357322039	5.96200004955739	0.851878960870608	17.7156928665296	0.881765178328303
7.98453623177242	0.855089679885419	9.05028334960135	0.852246914063562	13.4507758220403	0.891850180893491	5.97120405309834	0.856981780095856	17.8004305455201	0.886025959274449
7.98942312890788	0.858721799532047	9.05398927204534	0.854106556493021	13.5087101101325	0.894761310736851	5.97310710278678	0.858021857194142	17.8286253795314	0.887419096858376
7.99260995847721	0.861056842153949	9.05455380924679	0.854388456263952	13.5248037478224	0.895559841027709	5.97467756535521	0.858876299108449	17.8311673678687	0.887544098961311
7.9930382786713	0.861368664612531	9.05751829463626	0.855862748403733	13.5553468837317	0.897063232722689	5.98613831859193	0.865006111594281	17.9199676786876	0.891848778848113
7.99361667448884	0.861788986904998	9.06019527071015	0.857185380344777	13.6666009668669	0.902406388310016	5.98739855556435	0.865668834866195	17.9656049295818	0.894014366003578
7.99456498821534	0.862476248065403	9.06043326987447	0.85730257184629	13.7018560213528	0.904056376763682	6.00120786084862	0.872784485019358	18.1543030300741	0.902635916362426
7.99729771171744	0.864443641372723	9.06103264173717	0.857597416238313	13.7335841684537	0.905523679269204	6.00291554515126	0.873645852374728	18.1735785037232	0.903486769924134
7.99824932440348	0.865124195093373	9.06364349345747	0.858876942821148	13.7985990838251	0.908478555880183	6.00518919741379	0.874786378014968	18.1994028800978	0.904618124171904
8.00340979211325	0.868773901020281	9.07930543928716	0.866388673952633	13.8658262445869	0.911461368861188	6.00942904097159	0.876893953902269	18.3198348568493	0.909765449165586
8.00560973747185	0.870308869438439	9.09153772190587	0.872060903367706	13.895347287504	0.912748068741509	6.01446553412798	0.879365065803237	18.3493538458535	0.910995028389113
8.01365707518309	0.875817589615182	9.09368348213225	0.873038403925598	14.1098135969705	0.92167959290831	6.01857501937078	0.881355315584776	18.414162370009	0.9136507319181
8.01415484286952	0.876152872852544	9.09910097935379	0.875483174154718	14.3354822614347	0.930310453262396	6.0196404240074	0.881867489122621	18.422003801792	0.913967994100368
8.01432810186125	0.876269426758889	9.10740898491727	0.87916808049386	14.3402776049731	0.930485569515012	6.02828661585557	0.885966200915034	18.5010905445498	0.917119209399482
8.01475179755106	0.876554129565415	9.11305998017549	0.881630232507554	14.409674716185	0.932982035290192	6.03456589738704	0.888878688848211	18.5580066065113	0.919332736823221
8.01801409320442	0.878730867500104	9.12652649976143	0.887354090331472	14.4962876189814	0.935999863163663	6.03831485560166	0.890591947308897	18.6867858690867	0.924175933627442
8.01851683654855	0.879063903227182	9.13380086868083	0.890362481056495	14.5124577139916	0.936551383357973	6.03897212615651	0.890890351898478	18.6990540043214	0.924625511168805
8.02093952052402	0.880659753926949	9.13732319717495	0.891798266805148	14.5288859100475	0.937107911339041	6.03901141819047	0.890908172160719	18.7552076856287	0.926657419162294
8.02268752487112	0.881801917603749	9.14036067889053	0.893025507747647	14.6258127479951	0.940314380366957	6.04078160886211	0.891708844656758	18.7706435056727	0.927208552550566
8.02352896586061	0.882348958915358	9.1449869968349	0.89487534576046	14.7049612513054	0.942836504751073	6.04138493664607	0.891980766279537	18.7822335209015	0.927620283605679
8.02447426340215	0.882961379594705	9.1551032956544	0.898839462736095	14.7388590893833	0.943890692023967	6.04190471373678	0.892214636842895	18.7912808637467	0.927940445174079
8.03649434994743	0.890552307624873	9.15776830017415	0.899865390876063	14.7699743014746	0.944844791433319	6.0552595067987	0.898098969506686	18.8266349704477	0.929181130665449
8.03739708397507	0.891107785584288	9.15974647112676	0.900621987018243	14.7769796691336	0.945057822430663	6.05587704921773	0.898365298338555	18.9441840711049	0.933188483931177
8.03747669745479	0.891156676595513	9.16181802957941	0.90140981268551	14.80300287478	0.94584349068392	6.06350870384991	0.901614869956787	19.1281343856126	0.939104529560257
8.04144983943567	0.893576588191953	9.16208537978255	0.901511153481446	14.8425026968539	0.947019011815582	6.06953232036315	0.904125507579564	19.1689600819441	0.940360259540948
8.04184407715616	0.893814570058593	9.17465482811556	0.906189978396435	14.8562519102867	0.947423410176529	6.07165678208711	0.904999644728756	19.2252762778235	0.942059041925888
8.05068202278531	0.899049060377361	9.17605223358093	0.906699836298335	14.9728006179358	0.950753768744721	6.07342519337754	0.905722791357071	19.2424549330953	0.94256959659088
8.05116486975495	0.899329520351706	9.17982624146594	0.908066586613565	14.9908579693981	0.95125434343546	6.08045148686322	0.908555917580064	19.2515705914159	0.942839075632035
8.05608058229217	0.9021525047217	9.19591341579557	0.913726462212243	14.9923477896594	0.951295461037214	6.08729973930326	0.911256044924156	19.3520936316919	0.945745181894995
8.05651489756223	0.902399104234392	9.19781957482847	0.914379439985967	15.0384149858599	0.952553245270198	6.09597043772952	0.914588978177488	19.3873880870902	0.946737357284924
8.06742473612734	0.908444902311109	9.19987144905007	0.915078191070677	15.0572284963493	0.953059372124594	6.09845847625987	0.915527823144223	19.4397766686016	0.948183491652499
8.0719851688169	0.910888170675893	9.20248133140438	0.915960779930855	15.0955002576057	0.954075605268348	6.10328593326901	0.917327313932582	19.481824578824	0.949321460538864
8.08042758979171	0.915282618244884	9.20982622487037	0.918407641013557	15.1412469260383	0.955267044787467	6.10463311800394	0.917824306733828	19.7016033210249	0.95494922370524
8.08570080950361	0.917943754932922	9.21886192593333	0.921343614295378	15.1433055785515	0.955320070072961	6.10816886405568	0.919117979158443	19.8945207120563	0.959464278793151
8.08718869643564	0.918683105742045	9.2205130799361	0.921871362516353	15.2018182216482	0.956806145557311	6.11126707150702	0.920238872347438	19.9608908004825	0.960929933730424
8.08735409105601	0.918764981170175	9.23071563928035	0.925072938324434	15.2165752062024	0.957174563359368	6.11455210152753	0.92141447945283	19.9780462370585	0.961301678073045
8.09700508368183	0.923435563838428	9.23538131419767	0.926503255973316	15.2177675208837	0.957204219049091	6.11710324557479	0.922318355864094	19.9950132235009	0.961666499443129
8.11419320581448	0.931243955277368	9.25151436760047	0.931288420720956	15.4992568285575	0.963754417043016	6.11811397612896	0.92267426926356	20.0795487550305	0.963442599738899
8.11523381038417	0.931696212131525	9.26038387223244	0.933814817195796	15.5733611184622	0.965335095682263	6.12014829121037	0.923386864910155	20.1245873942819	0.964361024917361
8.12301929486994	0.935007355601124	9.26595193394951	0.935363682329012	15.592833915353	0.965740932794138	6.1254636921604	0.925225204151894	20.1463388670132	0.964797759281096
8.12847821212504	0.937253727759813	9.27593924589287	0.938071138103182	15.6802813827659	0.967515576501891	6.12855137438067	0.926277519922211	20.14774587905	0.96482585794796
8.1297694746778	0.937776135866373	9.28145936977327	0.939529142292424	15.6867897316189	0.967644566429646	6.13449715762248	0.928271969655909	20.242168450454	0.966669882099289
8.13345766560757	0.939249598300673	9.28228485006066	0.939744844870588	15.6898357810873	0.967704791180102	6.13748130400164	0.929257242023296	20.2786026145927	0.967359798713991
8.13690709147812	0.940602843013832	9.28641941402089	0.940816179426993	15.7147368545047	0.968193659510123	6.14292913650178	0.931029081674037	20.5486435566284	0.972114366434824
8.14764577400221	0.944664823778599	9.28780166674436	0.94117099320725	15.7498467796602	0.968872550889115	6.14515008405621	0.931741524550172	20.5696758412586	0.972459112550242
8.14949737383576	0.9453424931453	9.29068586088994	0.941905966988678	15.8227545310237	0.970244047822461	6.15637075084967	0.935254411553085	20.5847801347139	0.972704493167296
8.15466573026747	0.947199380175266	9.29124858935774	0.942048521220782	15.915192384375	0.971910479154463	6.18821179186582	0.944460799477408	20.5863585103359	0.972730029503556
8.15671072030184	0.947920139523965	9.29569774617997	0.943165952286781	16.0808444726808	0.974702336322634	6.18830498207699	0.94448614118428	20.6158925774071	0.973204193998385
8.15798729128068	0.948366091750271	9.29774719432797	0.943674941146032	16.0853038974817	0.974774158472538	6.18911854454493	0.944706990003693	20.6204818621883	0.973277252540789
8.16227759966588	0.949842639715201	9.30642129866447	0.945789511072723	16.3873620881388	0.97925646844342	6.206023422967	0.949140826126396	20.7494289345664	0.975262996193578
8.16723562937805	0.951506850185591	9.31684032324971	0.948245858624554	16.392916172914	0.979332121382878	6.20836226607478	0.949731323195509	20.9322693688283	0.977865326341446
8.17764363551629	0.954856713289708	9.32115424473106	0.949236631754726	16.5003141666395	0.980749688040896	6.20921309036278	0.949944773830318	20.9788683575255	0.978490327652849
8.19254181721215	0.959325052162178	9.32235836345133	0.949510467120946	16.5004431227393	0.980751339187878	6.2209312454921	0.952811657673273	21.0379867108803	0.979261717971891
8.1927466571816	0.95938389125487	9.34009337470519	0.953408915009231	16.5940949741469	0.981919093431517	6.23044836060596	0.955041884192203	21.0792490644941	0.979786127810213
8.20252941466753	0.962114463714546	9.34176984110025	0.953764578036809	16.6364169685473	0.982426667514439	6.23501087693764	0.956080553877131	21.0839909387509	0.979845666414574
8.20433485078789	0.96260164278872	9.34849054216358	0.95516854295177	16.8896742387688	0.985216688960747	6.24276536462988	0.957801413374387	21.1792100837941	0.981010120831121
8.20606000059589	0.963062364856519	9.36152714968347	0.957793958952087	16.8901102107988	0.985221142544851	6.24318059442266	0.957891999088107	21.2136209968633	0.981416622279104
8.21182025286856	0.964567203933005	9.37110823101417	0.959643024838107	16.9867429823639	0.986180225468444	6.24320845382381	0.957898071202036	21.4762189069092	0.98428154492928
8.21660313279047	0.965778173355814	9.38566593538159	0.962326112458654	17.0195563640351	0.986493455092531	6.24348697962511	0.957958738523748	21.4823707277805	0.984343843415709
8.22572537553904	0.967993492861392	9.41094609490517	0.966638428653663	17.0929713281258	0.987172139000684	6.24938982428725	0.959227912993538	21.5469988795174	0.984985619845863
8.22826330833944	0.968588325635819	9.41306886657647	0.96698123945481	17.118347883043	0.987399770976541	6.25675142427821	0.960766982516161	21.7023590880721	0.986436566759476
8.23629954554297	0.970411828868173	9.41470395608745	0.96724330990914	17.1357556492633	0.987553892223865	6.25755019954126	0.960931098446682	21.8986009068202	0.988095064738446
8.24448230563719	0.972177417602871	9.41856573197019	0.967855467767534	17.3048885171925	0.988968286021231	6.26158476920395	0.961751518204432	21.9501574067717	0.988500452381746
8.25064954179129	0.973449342987498	9.44501141053959	0.971798402893473	17.4686111485057	0.990202114447451	6.26440930449947	0.962317477847634	22.2337959509984	0.99052299429568
8.25620539645131	0.974553226397371	9.47995558062242	0.976383173197656	17.6921083372286	0.991691015393289	6.28185311434823	0.965663025862459	22.2718316347522	0.99076904443807
8.27130982285765	0.977361597688319	9.49200334940142	0.977810973570794	17.9982624247755	0.993406641410777	6.29604194018341	0.968200742655977	22.3352486076322	0.991166864063143
8.27406559220963	0.977844711725899	9.4996808496671	0.978682298366092	18.8657203297559	0.996692750657904	6.30512139803929	0.969741823877651	23.4381375467152	0.996050183818943
8.28578702064628	0.979803503619096	9.50603594193346	0.979381488837808	18.9382675311925	0.996885457253893	6.31857922913688	0.97191177604487	23.9854430233992	0.99742229901494
8.29734473292132	0.981589137470396	9.52382015462152	0.981235684223016	19.3264440259804	0.997754993310436	6.31936601071786	0.972034521598152	24.034963536415	0.997522172473042
8.31361174253104	0.983873375172323	9.54298358852308	0.983072929529445	19.4246393044318	0.997936819113743	6.3558913138044	0.977260206062892	24.1287708041561	0.997701823136028
8.31831110534168	0.984486254729617	9.55088326130094	0.983784256818786	19.5508674878018	0.998150898684981	6.3837695577477	0.980672002096204	24.1624728408674	0.997763428815913
8.3456108211043	0.987665376338428	9.61319722872053	0.988549985192655	19.6618813208792	0.99832226548248	6.38768358255395	0.981114279793815	24.2165395377938	0.99785913993544
8.37895769937193	0.99077007323198	9.62752114465951	0.989455044530171	20.0194202384381	0.998780530244622	6.54477911061118	0.993023559872388	24.6946351717668	0.998557090973947
8.39299823154644	0.991857386298355	9.64053029627534	0.990222363514562	20.024070918854	0.998785651193106	6.56988584632663	0.994122057885377	24.9420284858747	0.998830020711345
8.40031941929743	0.992378389734681	9.67526220695748	0.992036880187859	20.9910056180201	0.999510038599945	6.61051804653408	0.995577285020429	25.2464552622116	0.999100759165597
8.61651675371519	0.999149164798454	9.87752762217705	0.997829088571301	21.4955176571532	0.999702681078199	6.87874212987786	0.999459863891564	27.310763586703	0.99987030983935

